Additive relations in irrational powers

We investigate the interaction between raising to an irrational power and addition of real numbers. Thus, for a finite set $A$ of non-negative real numbers, let $A^{[c]} = \{a^c : a \in A\}$. When $k$ is a positive integer, $c$ is a real irrational number, and $A$ is a subset of an $N$-term arithmetic progression in $\mathbb{R}_{\geq 0}$ having cardinality at least a power of $\log{N}$, we prove that the $k$-fold sumset $|kA^{[c]}| \sim_k |A|^k/k!$ as $|A| \to \infty$. This result is uniform in $c$. When $A = \{1, \dots, N\}$ and $k = 2$, this result can be combined with existing works to show that $|A^{[c]} + A^{[c]}| \sim N^2/2$ as $N \to \infty$ whenever $c \in \mathbb{R} \setminus \{0, 1, 2\}$. The sumset lower bound follows from a bound on the number of equal sums of $r$ and $s \geq r$ elements of $A^{[c]}$ (by taking $r = s = k$). When $r = s = 2$ or $s > r$, our bound is optimal up to a power of $\log N$. This bound is proved using a functional transcendence theorem for certain endomorphisms of $\mathbb{R}_{>0}^n$, and innovations in the Pila--Wilkie counting theorem in $\mathbb{R}_{\exp}$ due to Binyamini, Novikov and Zak. In a different direction, we provide a Diophantine approximation criterion on $c$ that, when satisfied, ensures that a linear form in the $c$-th powers of multiplicatively independent integers does not vanish. The proof involves linear forms in logarithms. This provides a new proof of a fact, due to Bays--Kirby--Wilkie and Jones--Servi, that when $A$ is a multiplicatively independent set of positive integers, there are infinitely many effectively computable real numbers $c$ such that $A^{[c]}$ is linearly independent over $\mathbb{Q}$.

==> article/content/dissociated_sets.tex <==
%auto-ignore

\section{Proof of Theorem \ref{theorem/higher_energy_for_small_c} and Theorem \ref{theorem/c-th_powers_can_be_dissociated}}
\label{proof_of_higher_energy_theorem_for_small_c}

We will use the following linear forms in logarithms result.

\begin{theorem}
    Let $b_1, \dots, b_m$ be integers and $a_1, \dots, a_m$ positive integers, and put
    \begin{align*}
        \Lambda = b_1 \log(a_1) + \dots + b_m \log(a_m).
    \end{align*}
    Suppose $\abs{b_i} \leq 1$ and $\abs{a_i} \leq N$ for $i \in \{1, \dots, m\}$, and that $\Lambda$ doesn't vanish. Then
    \begin{align*}
        \abs{\Lambda} > \exp(-(16m)^{2(m + 2)}(\log{N})^m).
    \end{align*}
\end{theorem}
\begin{proof}
    This is \cite{Baker--Wustholz_logarithmic_forms_and_group_varieties}.
\end{proof}

We now prove the theorems stated in Section \ref{introduction/additive_energy/generalisations_and_dissociated_sets}. \\

\noindent\textbf{Proof of Theorem \ref{theorem/higher_energy_for_small_c}.}
The theorem will be proved if we can show that for all $\vec{a} \in \{-1, 0, 1\}^S$ satisfying
\begin{align*}
    \sum_{n \in S} a_n = 0
\end{align*}
the sum
\begin{align*}
    s(\vec{a}) = \sum_{n \in S} a_n n^c
\end{align*}
doesn't vanish unless $\vec{a} = 0$. Assume $\vec{a}$ is nonzero. For convenience, put $\exp(y) = 1 + y + R(y)$ for real $y$. By expanding the exponential function and using the reverse triangle inequality, one has
\begin{align*}
    \abs{\sum_{n \in S} a_n n^c} \geq
    c\abs{\sum_{n \in S} a_n \log{n}} -
    \abs{\sum_{n \in S} a_n R(c\log{n})}.
\end{align*}
By the linear forms in logarithms estimate
\begin{align*}
    \abs{\sum_{n \in S} a_n\log{n}} >
    \exp(-(16m)^{2(m + 2)}(\log{N})^m)
\end{align*}
where $m = \card{S}$. Here we use the fact that $\vec{a}$ and that $S$ is a multiplicatively independent set to make sure that the linear form doesn't vanish. If $y < 1$ we have $R(y) \leq y^2$ so that
\begin{align*}
    \abs{\sum_{n \in S} a_n R(c\log{n})} \leq
    c^2 m(\log{N})^2.
\end{align*}
It follows that if
\begin{align*}
    c < c_0(m, N) =
    m^{-1}(\log{N})^{-2}\exp(-(16m)^{2(m + 2)}(\log{N})^m)
\end{align*}
then the sum $s(\vec{a})$ doesn't vanish. This finishes the proof of the theorem. \\

\noindent\textbf{Proof of Theorem \ref{theorem/c-th_powers_can_be_dissociated}.}
We will use the same formulation as before in terms of the sum $s(\vec{a})$, but now the main term comes from a lower bound on the algebraic number
\begin{align*}
    \alpha = \sum_{n \in S} a_n n^r.
\end{align*}
Expanding the exponential function, 
\begin{align*}
    \abs{s(\vec{a})} \geq
    \abs{\alpha} -
    \abs{\sum_{n \in S} a_n n^r(\exp((c - r)\log{n}) - 1)}.
\end{align*}
Let $F = \Q(\alpha)$, so that
\begin{align*}
    [F : \Q] \leq \prod_{n \in S} [\Q(n^{1/q} : \Q)] \leq q^m.
\end{align*}
Each one of its conjugates takes the form
\begin{align*}
    \sum_{n \in S} a_n n^r\exp\bigg(\frac{2\pi ib_n}{q}\bigg)
\end{align*}
for a vector $\vec{b} \in ((\Z/\phi(q)\Z)^\ast)^S$. Since $\alpha$ is an algebraic integer, we have
\begin{align*}
    \prod_{\sigma \in M_F^\infty} \abs{\alpha^\sigma} \geq 1,
\end{align*}
this product being the constant term of a monic polynomial with integer coefficients. By bounding the conjugates trivially from above, one has
\begin{align*}
    \abs{\alpha} \geq \prod_{\sigma \in M^\infty_F \setminus \{\infty\}} \abs{\alpha^\sigma}^{-1} \geq (mN^r)^{1 - d} \geq
    (mN^r)^{1 - q^m}.
\end{align*}
For the other quantity, we use the inequality $\exp(y) - 1 \leq \exp(y)y$, valid for $y < 1$ to obtain
\begin{align*}
    \abs{\sum_{n \in S} a_nn^r (\exp((c - r)\log{n}) - 1)}
    &\leq
    \sum_{n \in S} n^r \exp((c - r)\log{n})(c - r)\log{n}
    \\ &\leq
    (c - r)mN^c\log{N}.
\end{align*}
It now follows that $s(\vec{a})$ is positive as soon as
\begin{align*}
    \abs{c - r} < m^{-q^m}N^{r(1 - q^m) - c}(\log{N})^{-1}.
\end{align*}
This finishes the proof of the theorem.

\subsection{Proof of Corollary \ref{corollary/powers_of_primes_are_additively_and_multiplicatively_dissociated}}
\label{proof_that_powers_of_primes_are_additively_and_multiplicatively_dissociated}

To begin with we will simplify the Diophantine condition in Theorem \ref{theorem/c-th_powers_can_be_dissociated} for the special case when $S$ is the primes, so $m = \pi(N)$. Just using $\pi(N) \leq N$ we have
\begin{align*}
    m^{-q^m}N^{-(a/q)(q^m - 1) - c}(\log{N})^{-1} >
    N^{-q^N - (a/q)(q^N - 1) - c - 1}.
\end{align*}
Now
\begin{align*}
    q^N + (a/q)(q^N - 1) + c + 1 \leq (1 + c)(q^N + 1) \leq 2(1 + c)q^N
\end{align*}
so that
\begin{align*}
    m^{-q^m}N^{-(a/q)(q^m - 1) - c}(\log{N})^{-1} &>
    \exp(-2(1 + c)q^N\log(N)) \\ &>
    \exp(-2(1 + c)q^{2N}).
\end{align*}
Therefore, if $c$ is a real number so that there exist $a$ and $q$ satisfying
\begin{align*}
    \abs{c - \frac{a}{q}} \leq \exp(-2(1 + c)q^{2N}),
\end{align*}
then the set $\{p^c : \textrm{$p \leq N$ prime}\}$ is dissociated.

Now let $(d_n)_{n \geq 1}$ be a sequence of nonnegative integers and let
\begin{align*}
    c = \sum_{n \geq 1} 10^{-d_n}, \quad \frac{a_N}{q_N} = 
    \sum_{n \leq N} 10^{-d_n}
\end{align*}
so $q_N = 10^{d_N}$. We have
\begin{align*}
    \abs{c - \frac{a_N}{q_N}} &= \sum_{n > N} 10^{-d_n} \\
    &\leq \sum_{n > d_{N + 1}} 10^{-n} \\
    &< 10^{1 - d_{N + 1}}.
\end{align*}
Choosing the sequence $(d_n)$ to satisfy, say
\begin{align}
\label{equation/d_n_definition}
    d_{n + 1} \geq 100^{1 + nd_n}
\end{align}
for every $n \geq 1$, we have that the set $\{p^c : \textrm{$p \leq N$ prime}\}$ is dissociated. Since $c$ does not depend on $N$, and there are uncountably many sequences $(d_n)$ satisfying (\ref{equation/d_n_definition}), this proves the corollary.

==> article/content/dissociated_sets_v2.tex <==
%auto-ignore

\section{Proof of Theorem \ref{theorem_B}}
\label{proof_of_theorem_B}

We will actually prove the following theorem.

\begin{theorem}
\label{theorem/lower_bound_on_linear_form_in_c-th_powers}
    Fix $A > 0$ and $s$ a positive integer. There exists an effective constant $c_8$ such that the following holds. For integers $N \geq 2$ and $q > 0$ let
    \begin{align*}
        \psi_N(q) =
        \exp(-2^{600s^4}
        \max\{c_8, q^s, s, \log{A}, \log{N}\}^{50s^2})
    \end{align*}
    Let $c \in (0, 1)$ and suppose there exist integers $a$ and $q > 0$ with
    \begin{align*}
        0 < c - \frac{a}{q} \leq \psi_N(q).
    \end{align*}
    Then for all $x_1, \dots, x_n \in [N]$ that are either
    \begin{enumerate}[(1)]
        \item multiplicatively independent, or
        \item such that if $r$ is rational and $x_i^r$ and $x_j^r$ are $\Q$-linearly dependent, then $i = j$ or $r$ is an integer,
    \end{enumerate}
    and for all $a_1, \dots, a_n$ of absolute value at most $A$ we have
    \begin{align*}
        \abs{a_1x_1^c + \dots + a_nx_n^c} \geq 
        \exp\bigg(-2^{500s^4}
        \max\left\{c_7, q^s, s, \log{A}, \log{N}, -\log\left(c - \frac{a}{q}\right)\right\}^{50s^2}
        \bigg).
    \end{align*}
\end{theorem}

\noindent\textbf{Proof of Theorem \ref{theorem/lower_bound_on_linear_form_in_c-th_powers}.}
Let $y = a_1x_1^c + \dots + a_sx_s^c$ denote the linear form. For convenience let $\eps = c - a/q$. In the course of the argument we shall decide how small $\eps$ should be. Let $R(x, \eps)$ denote the remainder term
\begin{align*}
    x^\eps = 1 + \eps\log{x} + R(x, \eps),
\end{align*}
which satisfies the estimate $R(x, \eps) \leq x^\eps \eps^2/2$. Writing $x_i^c = x_i^{a/q}x_i^\eps$ and expanding each term $x_i^\eps$ around zero gives
\begin{align*}
    y &= \sum_{i = 1}^s a_ix_i^{a/q} (1 + \eps \log{x_i} + R(x_i, \eps)) \\
    &=
    \alpha + \eps \Lambda + \sum_{i = 1}^s a_ix_i^{a/q}R(x_i, \eps),
\end{align*}
where
\begin{align*}
    \alpha = \sum_{i = 1}^s a_ix_i^{a/q}, \quad
    \Lambda = \sum_{i = 1}^s a_ix_i^{a/q}\log{x_i}.
\end{align*}
The idea of the proof is the following. If $\alpha$ doesn't vanish, then, being an algebraic integer with bounded conjugates, we can write down a lower bound for $\abs{\alpha}$. At the same time, we can make $\eps$ small enough that the lower bound on $\abs{\alpha}$ is much larger than the other terms contributing to $y$. On the other hand, if $\alpha$ vanishes then a positive lower bound on $\Lambda$ can be used since the remainder term has order $\eps^2$. In any case, we will need to use the estimate
\begin{align*}
    \abs{\sum_{i = 1}^s a_i x_i^{a/q} R(x_i, \eps)} \leq
    AN^{a/q + \eps}s\eps^2 = AN^c s\eps^2.
\end{align*}
\textbf{Case $\alpha$ is nonzero.} Using the reverse triangle inequality and the estimate
\begin{align*}
    \abs{\Lambda} \leq A N^{a/q} (\log{N}) s
\end{align*}
we have
\begin{align*}
    \abs{y} &\geq
    \abs{\alpha} - AN^{a/q}(\log{N})s\eps - AN^cs\eps^2 \\
    &\geq \abs{\alpha} - 2AN^{c + 1}s\eps,
\end{align*}
where we have removed the log factor to get a cleaner final result.

By the triangle inequality, the conjugates of $\alpha$ lie in the disc of radius $AN^c s$, and since $\alpha$ is an algebraic integer of degree at most $q^s$ we have
\begin{align*}
    1 \leq \abs{\alpha}(AN^cs)^{q^s}.
\end{align*}
It follows that if
\begin{align*}
    \eps < \frac{1}{4} (AN^c s)^{-q^s - 1}N^{-1}
\end{align*}
then
\begin{align}
\label{equation/completed_lower_bound_when_alpha_is_nonzero}
    \abs{y} > \frac{1}{2}(AN^cs)^{-q^s} \geq
    \frac{1}{2}\exp(-\max\{q^s, \log{A}, \log{N}, s\}^2)
\end{align}
It will be more convenient to take
\begin{align*}
    \eps < \exp(-6\max\{a^s, \log{A}, \log{N}, s, 2\log{2}\}),
\end{align*}
which is certainly small enough to imply the lower bound in (\ref{equation/completed_lower_bound_when_alpha_is_nonzero}).

\textbf{Case $\alpha$ is zero.} By \cite[Theorem 1.1]{Carr--O'Sullivan_on_the_linear_independence_of_roots}, $\alpha$ is nonzero if condition (2) of the theorem is satisfied, so we may assume that $x_1, \dots, x_n$ are multiplicatively independent. We need the following linear forms in logarithms estimate.

\begin{lemma}
    \label{lemma/linear_forms_in_logarithms_lemma}
    There exists an effective constant $c_3 > 1$ such that if we put
    \begin{align*}
        c_4(s, q, A) = 2^{500s^4}
        \max\{c_7, q^s, \log{A}, \log{N}\}^{50s^2}
    \end{align*}
    then the lower bound
    \begin{align*}
        \abs{\Lambda} > \exp(-c_4)
    \end{align*}
    holds.
\end{lemma}
\begin{proof}
    In the notation of the \cite[Theorem 1]{Fel'dman_an_improvement_of_the_estimate_of_a_linear_form_in_the_logarithms_of_algebraic_numbers} we have $m = s$, $n \leq q^s$, $H_0 \leq 2A^qN^a$ and $h \leq 2N$. The cited result states that $\abs{\Lambda} > \exp(-B)$ where
    \begin{align*}
        B = n(n + \log{H_0})(4^{6m^2 - 2m + 1}n^{1/2}(c + \log{h}))^{12m^2 + 4m - 3},
    \end{align*}
    for an effective absolute constant $c$. Taking $c_3 = \exp(c)$ and using the fact that $a/q < c$, we have
    \begin{align*}
        B &\leq q^s(q^s + \log(2A^qN^a))
        (4^{10s^2}q^{s/2}\log(2c_3N))^{20s^2}
        \\ &\leq
        q^{10s^3 + 2s}2^{400s^4}(q^s + \log(2A^qN^a))(\log{2c_3N})^{20s^2}
        \\ &\leq
        q^{10s^3 + 2s}2^{400s^4 + 1}\max\{q^s, \log(2A^qN^a)\}
        \max\{c_6, \log{N}\}^{20s^2} \\ &\leq
        2^{500s^4}
        \max\{q^s, \log(2A^qN^a), c_6, \log{N}\}^{40s^2} \\ &\leq
        2^{500s^4}
        \max\{c_7, q^s, \log{A}, \log{N}\}^{50s^2}
    \end{align*}
    which is the desired bound.
\end{proof}

We now return to the proof of Theorem \ref{theorem/lower_bound_on_linear_form_in_c-th_powers}, and in particular to the case $\alpha = 0$. Then Lemma \ref{lemma/linear_forms_in_logarithms_lemma} implies that
\begin{align*}
    \abs{y} \geq \exp(-c_4)\eps - AN^cs\eps^2.
\end{align*}
If we take
\begin{align*}
    \eps < \exp(-2^{600s^4}\max\{c_7, q^s, \log{A}, \log{N}\}^{50s^2})
\end{align*}
then we have the lower bound
\begin{align*}
    \abs{y} > \frac{1}{2} \exp(-c_4)\eps.
\end{align*}
Combining the two lower bounds from the cases where $\alpha$ is zero and nonzero, we have at least
\begin{align*}
    \abs{y} \geq \frac{1}{2}\exp\bigg(-2^{500s^4}
    \max\{c_7, q^s, s, \log{A}, \log{N}, -\log{\eps}\}^{50s^2}
    \bigg).
\end{align*}
Combining the two upper bounds on $\eps$, we can take
\begin{align*}
    \psi_N(q) =
    \exp(-2^{600s^4}
    \max\{c_8, q^s, s, \log{A}, \log{N}\}^{50s^2}).
\end{align*}
for an effective constant $c_8$.

\noindent\textbf{Q.E.D.}

\begin{lemma}
\label{lemma/Diophantine_approximation_lemma}
    Let $\psi_n(q)$ be a sequence of increasing functions. There exist uncountably many real numbers $c$ with the following property. For each positive integer $n$ there are coprime integers $a$ and $q > 0$ with
    \begin{align*}
        \abs{c - \frac{a}{q}} < \psi_n(q)^{-1}.
    \end{align*}
\end{lemma}
\begin{proof}
    Let $(d_m)$ be an increasing sequence of positive integers with at least $d_m \gg m$, and let
    \begin{align*}
        c = \sum_{m \geq 1} 2^{-d_m} =
        \frac{a}{q} + \sum_{m > n} 2^{-d_m}
    \end{align*}
    with $a$ and $q$ coprime. Then $q = 2^{d_n}$. We therefore require that
    \begin{align*}
        \abs{c - \frac{a}{q}} = \sum_{m > n} 2^{-d_m} \leq
        \sum_{m \geq d_{n + 1}} 2^{-m}
        = 2^{1 - d_{n + 1}}
    \end{align*}
    is smaller than $\psi_n(q)^{-1}$. To achieve this, let
    \begin{align*}
        d_{n + 1} = 2\psi_n(2^{d_n}) + n + e_n
    \end{align*}
    for each $n \geq 1$ and for some sequence $(e_n)$ of positive integers. Since there are uncountably many such sequences $(e_n)$, this proves the lemma.
\end{proof}

To prove Theorem \ref{powers_of_primes_are_dissociated}, we apply Lemma \ref{lemma/Diophantine_approximation_lemma} to the sequence of functions
\begin{align*}
    \rho_n(q)^{-1} = 
    \min_{A, N, s \leq n} \psi_{A, N, s}(q),
\end{align*}
which yields an uncountable set of real numbers $c$ satisfying the hypotheses of Theorem \ref{theorem/lower_bound_on_linear_form_in_c-th_powers}.

% \begin{corollary}
%     Let $N \geq 2$ and let
%     \begin{align*}
%         0 < c < \exp\left(-10^{15}(\log{N})^4\right).
%     \end{align*}
%     Suppose $x_1, x_2, x_3, x_4 \in [N]$ are multiplicatively independent. Then
%     \begin{align*}
%         \abs{x_1^c + x_2^c - x_3^c - x_4^c} > c^2.
%     \end{align*}
% \end{corollary}

==> article/content/dissociated_sets_v3.tex <==
%auto-ignore

\section{Proof of Theorem \ref{theorem_B} and \ref{powers_of_primes_are_dissociated}}
\label{proof_of_lower_bound_on_linear_forms_in_irrational_powers}

\begin{theorem}
    Let $A, X > 0$ be real and let $s, q$ be positive integers. There exists an effectively computable positive valued function $\psi(A, X, s, q)$ with the following property. If there exist $a, q > 0$ integers with
    \begin{align*}
        0 < c - a/q < \psi(A, X, s, q),
    \end{align*}
    then for all $x_1, \dots, x_s$ multiplicatively independent integers in $[1, X]$, and all $a_1, \dots, a_s$ integers in $[-A, A]$, the form
    \begin{align*}
        a_1 x_1^c + \dots + a_s x_s^c
    \end{align*}
    does not vanish.
\end{theorem}
\begin{proof}
    Let $\eps = c - a/q$. We need to show that if $\eps$ is small enough compared to $A, X, s$ and $q$, then the form
    \begin{align*}
        F = a_1 x_1^c + \dots + a_s x_s^c
    \end{align*}
    does not vanish.

    Let $R(x, \eps)$ denote the remainder term in
    \begin{align*}
        x^\eps = 1 + \eps\log{x} + R(x, \eps),
    \end{align*}
    which satisfies the estimate $R(x, \eps) \ll_X \eps^2$ for $x \in [1, X]$. Writing $x_i^c = x_i^{a/q}x_i^\eps$ and expanding each term $x_i^\eps$ around zero gives
    \begin{align*}
        F &= \sum_{i = 1}^s a_ix_i^{a/q} (1 + \eps \log{x_i} + R(x_i, \eps)) \\
        &=
        \alpha + \eps \Lambda + \sum_{i = 1}^s a_ix_i^{a/q}R(x_i, \eps),
    \end{align*}
    where
    \begin{align*}
        \alpha = \sum_{i = 1}^s a_ix_i^{a/q}, \quad
        \Lambda = \sum_{i = 1}^s a_ix_i^{a/q}\log{x_i}.
    \end{align*}
    The idea of the proof is the following. If $\alpha$ does not vanish, then, being an algebraic integer with bounded conjugates, we can write down a lower bound for $\abs{\alpha}$. At the same time, we can make $\eps$ small enough that the lower bound on $\abs{\alpha}$ is much larger than the other terms contributing to $F$. On the other hand, if $\alpha$ vanishes then a positive lower bound on $\Lambda$ can be used since the remainder term has order $\eps^2$. In any case, we will need to use the estimate
    \begin{align*}
        \abs{\sum_{i = 1}^s a_i x_i^{a/q} R(x_i, \eps)} \ll_{A, X, s} \eps^2.
    \end{align*}
    \noindent\textbf{Case $\alpha$ is nonzero.} Using the reverse triangle inequality and the estimate $|\Lambda| \ll_{A, X, s} 1$ we have
    \begin{align*}
        \abs{F} &\geq
        \abs{\alpha} + O_{A, X, s}(\eps).
    \end{align*}
    By the triangle inequality, the conjugates of $\alpha$ lie in the disc of radius $AXs$, and since $\alpha$ is an algebraic integer of degree at most $q^s$ we have
    \begin{align*}
        1 \leq \abs{\alpha}(AXs)^{q^s - 1}.
    \end{align*}
    In particular $|\alpha|$ is bounded below by a positive constant depending on $A, X, s, q$. Hence, taking $\eps$ small in terms of $A, X, s, q$, we find that $F$ is non-zero.
    
    \noindent\textbf{Case $\alpha$ is zero.} In this case we have 
    \begin{align*}
        |F| \geq \eps(|\Lambda| - O_{A, X, s}(\eps)).
    \end{align*}   
    By \cite[Theorem 1]{Fel'dman_an_improvement_of_the_estimate_of_a_linear_form_in_the_logarithms_of_algebraic_numbers}, we have $|\Lambda| \gg_{A, X, s, q} 1$. Thus we can again make sure $F$ does not vanish by taking $\eps$ small in terms of $A, X, s, q$.

    Finally, choose $\psi(A, X, s, q)$ small enough so that if $\eps < \psi$, then $F$ does not vanish in either case.
\end{proof}

\begin{lemma}
\label{lemma/Diophantine_approximation_lemma}
    Let $\psi(A, X, s, q)$ be a decreasing function of $q$. There exist uncountably many real numbers $c$ with the following property. For each triple of positive integers $A, X, s$, there are coprime integers $a$ and $q > 0$ with
    \begin{align*}
        \left|c - \frac{a}{q}\right| < \psi(A, X, s, q).
    \end{align*}
\end{lemma}
\begin{proof}
    For a positive integer $N$, let $f_N(q)$ be the minimum of $\psi(A, X, s, q)$ taken over $A, X, s \leq N$. Thus if there are $a$ and $q > 0$ with
    \begin{align*}
        \left|
        c - \frac{a}{q}
        \right| < f_N(q)
    \end{align*}
    for all $N$, then the same is true of $\psi(A, X, s, q)$.

    Let $(d_n)$ be an increasing sequence of positive integers with at least $d_n \gg n$, and let
    \begin{align*}
        c = \sum_{n \geq 1} 2^{-d_n} =
        \frac{a}{q} + \sum_{n > N} 2^{-d_n}
    \end{align*}
    with $a$ and $q$ coprime. Then $q = 2^{d_N}$. We therefore require that
    \begin{align*}
        \abs{c - \frac{a}{q}} = \sum_{n > N} 2^{-d_n} \leq
        \sum_{n \geq d_{N + 1}} 2^{-n}
        \geq  2^{1 - d_{N + 1}}
    \end{align*}
    is smaller than $f_N(q)$. To achieve this, define the sequence $(d_n)$ by
    \begin{align*}
         2^{d_{n + 1}} \geq \frac{2}{f_n(2^{d_n})} + e_n
    \end{align*}
    for each $n \geq 1$, and for some sequence $(e_n)$ of positive integers. Since there are uncountably many such sequences $(e_n)$, this proves the lemma.
\end{proof}

For each positive integer $k$, let $c_k$ be defined, as in the proof of Lemma \ref{lemma/Diophantine_approximation_lemma}, by choosing $d_{n + 1}$ to the smallest positive integer with
\begin{align*}
    2^{d_{n + 1}} \geq
    \frac{2}{f_n(2^{d_n})} + k.
\end{align*}
Then the real numbers $c_k$ are effectively computable. Indeed, since $f_n(q)$ is an effectively computable function, the proof of Lemma \ref{lemma/Diophantine_approximation_lemma} provides an algorithm to compute the digits of $c_k$. By varying $k$, one obtains infinitely many effectively computable examples. This proves Theorem \ref{powers_of_primes_are_dissociated}.

==> article/content/exponential_sums.tex <==
%auto-ignore

\section{Exponential sums}

\subsection{Circle method approach}

For $t$ real, let
\begin{align*}
    D(t) = \sum_{n \leq N} e(-n^c t).
\end{align*}
For each real $y$ and $\delta > 0$, let $f_{y, \delta}(x)$ be the inverse Fourier transform of $w((x - y)/\delta)$, where $w$ is supported in $[-1, 1]$ and $w(0) = 1$. If $\delta_N$ is chosen small enough that when
\begin{align*}
    x_1^c + x_2^c \neq x_3^c + x_4^c
\end{align*}
and $\vec{x} \in [N]^4$ then
\begin{align*}
    \delta < \abs{x_1^c + x_2^c - x_3^c - x_4^c},
\end{align*}
then we have
\begin{align*}
    \int_\R \abs{D(x)}^2 f_{y, \delta}(x) \; dx = \card\{(x_1, x_2) \in [N]^2 : x_1^c - x_2^c = y\}.
\end{align*}

\subsection{Exponential sums}

Let $Q \leq \card{S + S}$ where $S = \{n^c : n \in [N]\}$. Let $\{y_1, \dots, y_Q\}$ be the first $q$ elements of the sumset. Also let $\phi(q)$ denote the number of ways to write $y_q$ as a sum of $c$-th powers. One has the Fourier transform
\begin{align*}
    \hat{\phi}(\xi) = \frac{1}{Q}\sum_{q \leq Q} \phi(q) e_Q(-q\xi).
\end{align*}
If $Q = \card(S + S)$, then
\begin{align*}
    \hat{\phi}(\xi) = \frac{1}{Q}\sum_{n_1, n_2 \leq N} e_Q(-(n_1^c + n_2^c)\xi)
    = \frac{1}{Q} \bigg(\sum_{n \leq N} e_Q(-n^c\xi)\bigg)^2.
\end{align*}
We also have Fourier inversion
\begin{align*}
    \sum_{\xi \leq Q} \hat{\phi}(\xi)e_Q(q\xi) =
    \frac{1}{Q}\sum_{r \leq Q} \phi(r) \sum_{\xi \leq Q} e_Q((q - r)\xi) =
    \phi(q).
\end{align*}
We can now use the fact that
\begin{align*}
    \sum_{q \leq Q} \phi(q)^2 = 2N^2 + O(N(\log{N})^\alpha)
\end{align*}
with Fourier inversion.
\begin{align*}
    \sum_{q \leq Q} \abs{\phi(q)}^2 &=
    \sum_{q \leq Q} \sum_{\xi_1, \xi_2 \leq Q} 
    \hat{\phi}(\xi_1)\hat{\phi}(\xi_2)^c e_Q(q(\xi_1 - \xi_2))
    \\ &=
    \sum_{\xi_1, \xi_2 \leq Q} \hat{\phi}(\xi_1)\hat{\phi}(\xi_2)^c
    \sum_{q \leq Q} e_Q(q(\xi_1 - \xi_2))
    \\ &= Q\sum_{\xi \leq Q} \abs{\hat{\phi}(\xi)}^2
    \\ &= \frac{1}{Q} \sum_{\xi \leq Q} \abs{\sum_{n \leq N} e_Q(-n^c\xi)}^4.
\end{align*}
This proves the following.

\begin{proposition}
    Let $N$ be a positive integer, $S = \{n^c : n \in [N]\}$, $Q = \card(S + S)$. Then
    \begin{align*}
        \sum_{\xi \leq Q} 
        \abs{\sum_{n \leq N} e_Q(-n^c \xi)}^4
        = 
        2N^2Q + O(NQ(\log{N})^\alpha).
    \end{align*}
\end{proposition}

\begin{corollary}
    \begin{align*}
        \card\{a \leq Q : \abs{D(a/Q)} \geq V\} \ll \bigg(\frac{N}{V}\bigg)^4.
    \end{align*}
\end{corollary}

==> article/content/final_remarks.tex <==
%auto-ignore

\section{Final remarks}
\label{final_remarks}

% We can also give an elementary argument showing that $2N^2$ cannot be the main term in an asymptotic for $E(S)$. There are $\gg N$ coprime pairs $1 \leq y_1^\ast, y_3^\ast \leq N^{1/2}$ of odd integers; $\gg N^{1/2}$ odd integers $d_1 \leq N^{1/2}/2$; $\gg N^{1/2}$ odd integers $2 \leq d_2 \leq N^{1/2}$; and setting
% \begin{align*}
%     \vec{x} = \bigg(
%     \frac{d_1y_1^\ast + d_2y_3^\ast}{2},
%     \frac{d_3y_1^\ast - d_1y_3^\ast}{2},
%     \frac{d_2y_3^\ast - d_1y_1^\ast}{2},
%     \frac{d_1y_3^\ast + d_2y_1^\ast}{2}
%     \bigg)
% \end{align*}
% gives $B(2, N) \gg N^2$. 

% We now describe the a family of irrational numbers $c$ for which (\ref{equation/additive_energy_of_c-th_powers}) admits a nontrivial solution, as promised in the introduction.

% Let $n > 1$, let $\phi_n$ be the unique root $\phi_n > 1$ of the polynomial
% \begin{align*}
%     x^{2n} - x^{n + 1} - x^n + 1,
% \end{align*}
% and let $c_n = \log_2(\phi_n)$. Then we have a nontrivial solution to (\ref{equation/additive_energy_of_c-th_powers})
% \begin{align*}
%     (2^{2n})^{c_n} + 1^{c_n} = (2^{n + 1})^{c_n} + (2^n)^{c_n}.
% \end{align*}
% This sequence $(c_n)$ tends to zero, and so the probabilistic heuristic that (\ref{equation/additive_energy_of_c-th_powers}) admits fewer solutions as $c$ grows isn't able to take effect.

If we instead let $\phi_n$ be a root of the polynomial $x^{2n} - 2x^{n + 1} + 1$, and let $c_n = \log_2(\phi_n)$ again, then $1, 2^{n + 1}, 4^n$ will form a 3-term arithmetic progression in the $S$.

In a different direction to Theorem \ref{theorem/main_theorem} and Theorem \ref{theorem/theorem_on_additive_energy_with_effective_implied_constants}, one can think of the real exponent $c$ as varying. Through these considerations, one observes that the equation (\ref{equation/additive_energy_of_c-th_powers}) has no nontrivial solutions for almost all $c$. This can be argued as follows. If $\vec{a} = (a_1, \dots, a_4) \in [N]^4$ does not satisfy $a_1 \in \{a_3, a_4\}$, then the function $f_{\vec{a}}(c) = a_1^c + a_2^c - a_3^c - a_4^c$ does not vanish identically. Therefore, for example because it can be extended to an analytic function on a disc, its zeros are countable, and hence form a set of measure zero. As $\vec{a}$ varies, the numbers $c$ such that $f_{\vec{a}}(c) = 0$ vary over a countable union of sets of measure zero.

\comment{Question: does $f_{\vec{a}}$ always have exactly one or two zeros? What is the ``one zero locus'' of $\vec{a} \in \R_{> 0}^4$?}

==> article/content/introduction/acknowledgements.tex <==
%auto-ignore

\renewcommand{\abstractname}{{\sc Acknowledgements}}
\begin{abstract}
The author would especially like to thank Harry Schmidt for helpful conversations and guidance, without whom this paper would not exist. Additional thanks are owed to Sam Chow and Akshat Mudgal for introducing us to the problem, to Nathan Lockwood for conversations regarding the construction of non-trivial solutions, and to Gareth Jones for showing us the Schanuel result of Bays--Kirby--Wilkie and for remarks about effectivity in the result of Binyamini--Novikov--Zak. Joseph Harrison is supported by the Warwick Mathematics Institute Centre for Doctoral Training, and gratefully acknowledges the funding from the UK Engineering and Physical Sciences Research Council (Grant number: \texttt{EP/W524645/1}).
\end{abstract}

==> article/content/introduction/multiplicatively_independent_solutions.tex <==
%auto-ignore

\subsection{Multiplicatively independent solutions}

\subsubsection{Construction of 3AP and sporadic solutions}
\label{introduction/construction_of_3AP_and_sporadic_solutions}
\textbf{I would put this whole discussion after the proofs of Theorem 2 and 3 }

We would like to point out two features of these solutions. First, the sequence $c_n$ has polynomial decay, but the solutions grow exponentially. Moreover, the solutions constructed are \define{multiplicatively dependent}; i.e., there are relations of the form
\begin{align*}
    x_1^{a_1} x_2^{a_2} x_3^{a_3} x_4^{a_4} = 1
\end{align*}
in the coordinates of $\vec{x}$, where $\vec{a} \in \Z^4$. If $\vec{x}$ is a solution obtained via a polynomial
\begin{align*}
    x^a + x^b - x^c - 1
\end{align*}
as above, we can choose integers $a_1$ and $a_2$ so that $a_1 a + a_2 b = c\gcd(a, b)$, in which case
\begin{align*}
    x_1^{a_1}x_2^{a_2}x_3^{-\gcd(a, b)} = 1
\end{align*}
is a nontrivial multiplicative relation. This prompts the following question, which we will state in a more general context.
\subsubsection{Generalisations and dissociated sets}
\label{introduction/additive_energy/generalisations_and_dissociated_sets}

Question \ref{question/multiplicatively_independent_solutions_to_generalised_equation} can be stated in the language of dissociated sets. Recall that a subset $S$ of an additive abelian group $A$ is called \define{dissociated} if all sums of distinct elements of $S$ are different, i.e., whenever $\{x_1, \dots, x_n\}$ and $\{y_1, \dots, y_m\}$ are subsets of $S$ of cardinality $n$ and $m$, such that
\begin{align*}
    x_1 + \dots + x_n = y_1 + \dots + y_m
\end{align*}
one has $n = m$ and $\{x_1, \dots, x_n\} = \{y_1, \dots, y_m\}$. In particular, a negative answer to Question \ref{question/multiplicatively_independent_solutions_to_generalised_equation} is equivalent to the assertion that $\{n^c : n \in S\}$ is dissociated, as $S$ ranges over all finite multiplicatively independent sets of positive integers. The following result is a partial strengthening, as it allows $S$ to be countably infinite. 

\begin{section_indexed_theorem}
    There exist uncountably many, effectively computable real numbers $c$, such that if $x_1^c, \dots, x_n^c$ are $\Q$-linearly dependent, then $x_1, \dots, x_n$ are multiplicatively dependent.
\end{section_indexed_theorem}

The term ``effectively computable'' is used in the standard sense that there exists an algorithm that, given an $\eps > 0$, returns a rational number $r$ satisfying $\abs{c - r} < \eps$ after a finite number of steps. 

Continuing the theme of additive combinatorics, we can derive some consequences in the theory of dissociated sets. 

\begin{corollary}
    There are uncountably many real numbers $c$ such that for any multiplicatively independent set of positive integers $S$, the set $\{s^c : s \in S\}$ is additively dissociated. In particular, the set $\{p^c : \textrm{$p$ prime}\}$ is both additively and multiplicatively dissociated, for uncountably many real $c$.
\end{corollary}

\begin{theorem}
    \label{theorem/theorem_on_dissociated_sets}
    There exists an uncountable set of effectively computable, real transcendental numbers $c$ with the following property. Let $S$ be a set of positive integers, and assume that either
    \begin{enumerate}[(1)]
        \item the set $S$ is multiplicatively independent or
        \item that nonintegral, rational powers of elements in $S$ are pairwise $\Q$-linear independent.
    \end{enumerate}
    Then the set $\{s^c : s \in S\}$ is dissociated.
\end{theorem}

In particular, this answers Question \ref{question/multiplicatively_independent_solutions_to_generalised_equation} negatively for an uncountable set of real numbers $c$. We remark that the complement of this uncountable set of $c$ is unfortunately also uncountable. Theorem \ref{theorem/theorem_on_dissociated_sets} will be proved in Section \ref{proof_of_theorem_on_dissociated_sets}.

This theorem has applications to the construction of dissociated sets of real numbers. Countable dissociated subsets of $\R$ must exist by measure theoretic considerations. For example, a countable subset $S \subseteq \R$ can be regarded as an element $(x_i)$ of the space $\R^\infty$ of all real sequences indexed by positive integers. This space can be equipped with a measure, so that the hyperplanes
\begin{align*}
    \sum_{i \in T_1} x_i = \sum_{i \in T_2} x_i
\end{align*}
have measure zero for every choice of distinct finite subsets $T_1$ and $T_2$ of positive integers. Since there are countably many hyperplanes, their complement in $\R^\infty$ must be nonempty.

It is not clear how one can use this argument to effectively compute dissociated sets in $\R$. Our Theorem \ref{theorem/theorem_on_dissociated_sets} has the following corollary, which provides an effectively computable example of a countable set of real numbers, which is both additively and multiplicatively dissociated.

\begin{corollary}
    \label{corollary/c-th_powers_of_primes_are_dissociated}
    For uncountably many, effectively computable real numbers $c$, the set $\{p^c : \textrm{$p$ prime}\}$ is dissociated.
\end{corollary}

==> article/content/introduction/rational_exponents.tex <==
%auto-ignore

\subsection{Rational exponents}
\label{introduction/rational_exponents}

We now explain how to prove Theorem \ref{theorem/sumset_asymptotic} when $c$ is rational.

\subsubsection{Previous work}
\label{introduction/previous_work}

The analogue of Theorem \ref{theorem/main_theorem} with $c$ replaced with a positive integer $d$ has received plenty of attention over the years.

When $d = 2$, sporadic solutions really do make a contribution. We use the Vinogradov notation, so that $f(x) \gg g(x)$ if $g(x) = O(f(x))$. Now there are $\gg N$ coprime pairs $1 \leq y_1^\ast, y_3^\ast \leq N^{1/2}$ of odd integers; $\gg N^{1/2}$ odd integers $d_1 \leq N^{1/2}/2$; $\gg N^{1/2}$ odd integers $2 \leq d_2 \leq N^{1/2}$; and setting
\begin{align*}
    \vec{x} = \bigg(
    \frac{d_1y_1^\ast + d_2y_3^\ast}{2},
    \frac{d_3y_1^\ast - d_1y_3^\ast}{2},
    \frac{d_2y_3^\ast - d_1y_1^\ast}{2},
    \frac{d_1y_3^\ast + d_2y_1^\ast}{2}
    \bigg)
\end{align*}
gives $B(2, N) \gg N^2$. By considering the arithmetic function
\begin{align*}
    r(n) = \card\{(x_1, x_2) \in [N]^2 : x_1^2 - x_2^2 = n\},
\end{align*}
which has $r(0) = N$ and $r(n) \ll_\eps n^\eps$ for $n \neq 0$, we see that the total number of solutions to $(\ref{equation/additive_energy_of_c-th_powers})$ when $c = 2$ is $\ll N^2(\log{N})^3$. Here we have used a second moment estimate on the divisor function, which can be found in \cite{Luca--Toth_the_r-th_moment_of_the_divisor_function}, and was known to Ramanujan \cite{Ramanujan_some_formulae_in_the_analytic_theory_of_numebrs}.

Hooley addressed the case $d = 3$ in \cite{Hooley_on_the_representations_of_a_number_as_a_sum_of_two_cubes, Hooley_on_the_numbers_that_are_representable_as_the_sum_of_two_cubes} and arbitrary $d$ in \cite{Hooley_on_the_representation_of_a_number_as_the_sum_of_two_h-th_powers, Hooley_on_another_sieve_method_and_the_numbers_that_are_a_sum_of_two_h-th_powers}. Greaves \cite{Greaves_on_the_representation_of_a_number_as_a_sum_of_two_fourth_powers} improved Hooley's result for $d = 4$ and Skinner--Wooley \cite{Skinner--Wooley_sums_of_two_kth_powers} obtained an improvement for $d \geq 5$ using the Bombieri--Pila determinant method. The further improvements of Heath-Brown \cite{Heath-Brown_the_density_of_rational_points_on_curves_and_surfaces} and Browning \cite{Browning_equal_sums_of_two_kth_powers} for $d \geq 6$ also use the determinant method, together with geometric insights that allow for clever choices of plane sections. Recently, Salberger \cite{Salberger_counting_rational_points_on_projective_varieties} has shown that $N_1(d, N) \ll_d N^{3/d^{1/2}}(\log{N})^4$. In particular, there is a $\delta > 0$ so that for every positive integer $d \geq 3$, one has $N_1(d, N) \ll N^{2 - \delta}$, and this is enough to establish Theorem \ref{theorem/sumset_asymptotic} for positive integers not equal to $1$ or $2$. There is also the folklore conjecture, stated in \cite{Hooley_on_the_representation_of_a_number_as_the_sum_of_two_h-th_powers}, that $B(d, N) = 0$ if $d \geq 5$. 

These remarks can be ``explained'' in terms of the Diophantine geometry of the surface $X_d \subseteq \P^3_\Q$ defined by (\ref{equation/additive_energy_of_c-th_powers}) when $c = d$. The surface $X_3$ is rational over $\Q$, and so there are many nontrivial rational points. In particular, they are Zariski dense in $X_3$. The surface $X_4$ is K3 and admits an elliptic fibration with generic fibre having Mordell--Weil rank one. In this case, the nontrivial solutions are accounted for by jumps in the Mordell--Weil ranks of fibres, and it is known that the subset of $\Q$-points on the base where the rank jumps is not a thin set. That the rational points of $X_4$ are Zariski dense is proved in \cite{Swinnerton-Dyer_A4+B4=C4+D4_revisted}. Finally, the surfaces $X_d$ for $d \geq 5$ are of general type, and the conjecture that $X_d$ contains no nontrivial rational points can be regarded as a manifestation of the Bombieri--Lang conjecture, wherein the rational points of $X_d$ are not Zariski dense, in contrast to the cases $d \in \{3, 4\}$.

We now address the case of rational, nonintegral exponents $c$.

\begin{theorem}
    \label{theorem/additive_energy_in_the_rational_case}
    For $0 < \eps < (\log_2{N})^{-1}$ let
    \begin{align*}
        \alpha =
        \bigg(
        \frac{1}{\log_2{N}} - \eps
        \bigg)
        \begin{cases}
            q - a & a \in \{1, 2\}, \\
            q - 3a^{-1/2} & a > 2,
        \end{cases} 
        \\
        \beta =
        \frac{1}{q}
        \begin{cases}
            a & a \in \{1, 2\}, \\
            a^{-1/2} & a > 2,
        \end{cases}
        \quad\quad\quad
        \gamma =
        \begin{cases}
            0 & a = 1, \\
            3 & a = 2, \\
            4 & a > 2. \\
        \end{cases}
    \end{align*}
    Then
    \begin{align*}
        B(1/q, N) = \frac{N^{1 - \alpha}}{1 - 1/q}
        + \zeta(1/q)N^\beta + O_q(N^{-\eps}),
    \end{align*}
    and when $a > 1$
    \begin{align*}
        B(a/q, N) \ll_{a, q} (N^{1 - \alpha} + N^\beta)(\log{N})^\gamma.
    \end{align*}
\end{theorem}

Theorem \ref{theorem/additive_energy_in_the_rational_case} will be proved in Section \ref{proof_of_additive_energy_theorem_in_rational_case}. Note that the term $N^{1 - \alpha}$ dominates if and only if $N > 2^{1/(1/q + \eps)}$, and so in particular it dominates when $N > 2^q$.

Together with the remarks in Section \ref{introduction/previous_work}, this reduces the proof of Theorem \ref{theorem/sumset_asymptotic} to the case when $c$ is irrational.


==> article/content/introduction/sumset_result.tex <==
%auto-ignore

\section{Introduction}

Our main theorem is the following. 

\begin{manualtheorem}{A}
\label{sumset_theorem}
    Let $c \not \in \{0, 1, 2\}$ be a real number, let $N$ be a positive integer, and let
    \begin{align*}
        S = \{1^c, 2^c, \dots, N^c\}.
    \end{align*}
    Then the cardinality of the sumset $S + S$ is asymptotic to $N(N + 1)/2$ as $N \to \infty$.
\end{manualtheorem}

It is clear that the conclusion of Theorem \ref{sumset_theorem} does not hold when $c \in \{0, 1\}$. If $c = 2$, a theorem of Landau \cite{Landau_on_the_partition_of_positive_integers_in_four_classes_according_to_the_minimal_number_of_squares_needed_to_their_additive_composition} implies that $\card(S + S) \ll N^2(\log{N})^{-1/2}$. We note that Theorem \ref{sumset_theorem} improves on \cite[Corollary 3.2]{Elekes--Nathanson--Ruzsa_convexity_and_sumsets} for the convex function $f(x) = x^c$ when $A = [N]= \{1, \dots, N\}$.

A standard argument involving the Cauchy--Schwartz inequality, which can be found in \cite[Lemma 2.9, Corollary 2.10]{Tao--Vu_additive_combinatorics}, reduces the proof of Theorem \ref{sumset_theorem} to an estimate
\begin{align*}
    \card\{\vec{x} \in [N]^4: x_1^c + x_2^c = x_3^c + x_4^c\}
    = 2N^2 + o(N^2)
\end{align*}
for the so-called additive energy of the set $S$. When $c \not \in \{0, 1, 2\}$ is rational, such an estimate follows from \cite{Salberger_counting_rational_points_on_projective_varieties} and \cite{Carr--O'Sullivan_on_the_linear_independence_of_roots}. We explain this in Section \ref{section:rational_case}. The main contribution of this paper handles the irrational exponents.

\begin{manualtheorem}{B}
\label{irrational_additive_energy_theorem}
    Let $N$ be a positive integer and let $c$ be a real irrational number. There exists a positive integer $\alpha$ such that
    \begin{align*}
        \card\{\vec{x} \in [N]^4 : x_1^c + x_2^c = x_3^c + x_4^c\}
        = 2N^2 + O(N(\log{N})^\alpha).
    \end{align*}
    Moreover, $\alpha$ and the big-O constant are effectively computable, and do not depend on $c$ or $N$.
\end{manualtheorem}

% The product set $S \cdot S$ is in bijection with the product set $[N] \cdot [N]$, and the problem of determining the cardinality of this latter set is known as the Erd\H{o}s multiplication table problem \cite{Erdos_on_an_asymptotic_inequality_in_number_theory}. The true order of magnitude of this cardinality was determined in \cite[Corollary 3]{Ford_the_distribution_of_integers_with_a_divisor_in_a_given_interval} to be
% \begin{align*}
%     \frac{N^2}{(\log{N})^\delta (\log\log{N})^{3/2}} \ll
%     \card([N] \cdot [N]) \ll \frac{N^2}{(\log{N})^\delta (\log\log{N})^{3/2}},
% \end{align*}
% where $\delta = 1 - (1 + \log\log{2})/\log{2}$ is the Erd\H{o}s--Ford--Tenenbaum constant. In conjunction with our Theorem \ref{theorem/sumset_asymptotic}, this may be interpreted as saying that the sets $S$ admit very little additive or multiplicative structure when $c$ is a real number, not equal to $0, 1$ or $2$.

A key ingredient in establishing Theorem \ref{irrational_additive_energy_theorem} is a recent o-minimal point counting theorem \cite{Binyamini--Novikov--Zak_Wilkie's_conjecture_for_Pfaffian_structures}. This result is a development of the celebrated Pila--Wilkie theorem \cite{Pila--Wilkie_the_rational_points_on_a_definable_set}, and answers a question \cite[Conjecture 1.11]{Pila--Wilkie_the_rational_points_on_a_definable_set} known as Wilkie's conjecture. We note that applying \cite{Pila--Wilkie_the_rational_points_on_a_definable_set} delivers an error term $O(N^{1 + \eps})$, which is already sufficient for proving Theorem \ref{sumset_theorem}.

Another ingredient in our argument is the classical Ax--Schanuel theorem for the exponential function \cite{Ax_on_Schanuel's_conjectures}. In Proposition \ref{proposition/functional_transcendence_proposition}, we use this theorem to prove a functional transcendence statement for irrational powers that may be considered interesting in its own right.

% Let $Z$ be a semi-algebraic subset of $\R_{>0}^n$ and $c$ an irrational number. then the set $\{(x_1^c, \dots, x_n^c) : \vec{x} \in Z\}$ is Zariski dense in $\R_{>0}^n$.

In \cite{Chapman--Chow--Holdridge_additive_Ramsey_theory_over_Piatetski-Shapiro_numbers}, a result \cite[Theorem 2]{Robert--Sargos_three-dimensional_exponential_sums_with_monomials} concerning a Diophantine inequality resembling the additive energy equation in Theorem \ref{irrational_additive_energy_theorem} is applied to the question of partition regularity of linear relations in the Piatetski--Shapiro sequence $\floor{n^c}$. The question of proving an asymptotic formula like the one appearing in Theorem \ref{irrational_additive_energy_theorem} was brought to our attention by Sam Chow and Akshat Mudgal.

In Theorem \ref{irrational_additive_energy_theorem}, we regard the real number $c$ as fixed, and count the number of solutions to a particular instance of the equation
\begin{align}
    \label{additive_energy_equation}
    x_1^c + x_2^c = x_3^c + x_4^c.
\end{align}
We now let $c$ vary, investigating the properties of the set of $c$ for which equation (\ref{additive_energy_equation}) admits non-trivial solutions. Since each $\vec{x} \in \Z_{>0}^4$ is a solution of at most countably many (in fact finitely many) equations of the form (\ref{additive_energy_equation}), the set of real numbers $c$ so that (\ref{additive_energy_equation}) admits a non-trivial solution is countable, being a union over $\Z_{>0}^4$ of countable (in fact finite) sets.

%% Why is this clear? Does this mean that the set is infinite? 

%hopefully clear now. it isn't clear that the set is infinite from this, I think. It does follow from the example below showing the set is not discrete.

Let $(x_1, x_2, x_3, x_4)$ be a non-trivial solution to (\ref{additive_energy_equation}), and assume without loss of generality that $x_1 \geq x_2$ and $x_1 > x_3 \geq x_4$. Then the inequality
\begin{align*}
    x_1^c \leq x_1^c + x_2^c = x_3^c + x_4^c \leq 2x_3^c
\end{align*}
implies $c \leq (\log{2})N$. Thus if $c > (\log{2})N$, then (\ref{additive_energy_equation}) admits no non-trivial solutions at all.

Let $\phi$ be a zero of the polynomial $x^{2n} - x^{n + 1} - x^n + 1$, and let $c = \log_2(\phi)$. Then $(2^{2n}, 1, 2^{n + 1}, 2^n)$ is a non-trivial solution to (\ref{additive_energy_equation}). Since $c \to 0$ as $n \to \infty$, this construction shows that the set of real numbers $c$ so that (\ref{additive_energy_equation}) admits non-trivial solutions is not discrete, and contains infinitely many irrational members.

We can say more under an additional assumption that the coordinates $x_1, x_2, x_3, x_4$ of a non-trivial solution to (\ref{additive_energy_equation}) are multiplicatively independent. Suppose the numbers $\log{x_1}, \dots, \log{x_4}$ are $\Q(c)$-linearly independent. This condition is satisfied if $c$ is algebraic by Baker's theorem \cite{Baker_linear_forms_in_the_logarithms_of_algebraic_numbers}. If Schanuel's conjecture holds for the numbers $\log{x_1}, \dots, \log{x_4}, c\log{x_1}, \dots, c\log{x_4}$, then the inequality
\begin{align*}
    \trdeg_{\Q}(c, x_1^c, \dots, x_4^c) \geq 4
\end{align*}
holds. Thus if $c$ is algebraic, Schanuel's conjecture implies that all solutions of (\ref{additive_energy_equation}) are multiplicatively dependent.

A real number $c$ is called exponentially algebraic if it is a coordinate of a smooth solution of a system of polynomial equations in variables $y_1, \dots, y_n$ and their exponentials $\exp(y_1), \dots, \exp(y_n)$. In \cite[Theorem 1.1]{Bays--Kirby--Wilkie_A_Schanuel_property_for_exponentially_transcendental_powers}, the authors show that if $c$ is exponentially transcendental, then
\begin{align*}
    \trdeg_{\Q(c)}(y_1, \dots, y_n, y_1^c, \dots, y_n^c)
    \geq n
\end{align*}
for any $y_1, \dots, y_n \in \R_{>0}$. In particular, if $c$ is exponentially transcendental then all solutions to (\ref{additive_energy_equation}) are multiplicatively dependent. In \cite[Section 4]{Jones--Servi_on_the_decidability_of_the_real_field_with_a_generic_power_function}, a computable example of an exponentially transcendental number is given. We thank Gareth Jones for these remarks.

We prove a Diophantine approximation criterion that ensures non-trivial solutions of (\ref{additive_energy_equation}) are multiplicatively dependent. We state our result for an arbitrary integer linear combination of irrational powers.

\begin{manualtheorem}{C}
\label{theorem_B}
    Let $A, X > 0$ be real and let $s, q$ be positive integers. There exists a positive valued function $\psi = \psi(A, X, s, q)$ with the following property. If there exist $a, q > 0$ integers with
    \begin{align*}
        0 < c - a/q < \psi(A, X, s, q),
    \end{align*}
    then for all $x_1, \dots, x_s$ multiplicatively independent integers in $[1, X]$, and all $a_1, \dots, a_s$ integers in $[-A, A]$, the form
    \begin{align*}
        a_1 x_1^c + \dots + a_s x_s^c
    \end{align*}
    does not vanish.
\end{manualtheorem}

Theorem \ref{theorem_B} is proved in Section \ref{proof_of_theorem_B}. Besides the use of an effective linear forms in logarithms result of Fel'dman \cite{Fel'dman_an_improvement_of_the_estimate_of_a_linear_form_in_the_logarithms_of_algebraic_numbers}, the proof is elementary.

The function $\psi(A, X, s, q)$ arises from lower bounds for linear forms in logarithms, and so it decreases extremely rapidly. Examining the proof of Theorem \ref{theorem_B} and appling the Borel--Cantelli lemma shows that the set of real numbers $c$ satisfying the Diophantine approximation condition
\begin{align*}
    0 < c - a/q < \psi(A, X, s, q)
\end{align*}
has Lebesgue measure zero. It is easy to see (Lemma \ref{lemma/Diophantine_approximation_lemma}) that uncountably many real numbers $c$ do satisfy this condition. The proof of Lemma \ref{lemma/Diophantine_approximation_lemma} supplies effectively computable examples of such real numbers $c$. We therefore have the following.

\begin{manualtheorem}{D}
    \label{powers_of_primes_are_dissociated}
    There exist infinitely many real numbers $c$, whose digits can be effectively computed, such that $\{p^c : \textrm{$p$ prime}\}$ is linearly independent over $\Q$. %Moreover the set of $c$ such that $\{p^c : \textrm{$p$ prime}\}$ is linearly independent is uncountable.  
\end{manualtheorem}
We remark that Theorem \ref{powers_of_primes_are_dissociated} trivially implies that there is an effectively computable $c$ such that the set of prime powers $p^c$ is additively dissociated. This is a property of interest in additive combinatorics and the main motivation for proving Theorem \ref{powers_of_primes_are_dissociated}. 
%It follows from considering

\begin{notation}
    Throughout this paper, we will use the Bachmann--Landau notation, so we write $f(x) = O_{A, B, \dots}(g(x))$ if $f$ and $g$ are real-valued functions with $\abs{f(x)} \leq c_1 g(x)$ for some constant $c_1$ depending on $A, B, \dots$, and for a set of $x$ that will be clear from the context. We also use the Vinogradov  notation $f(x) \ll_{A, B, \dots} g(x)$ if $f(x) = O_{A, B, \dots}(g(x))$. We call the constant $c_1$ the ``big-$O$ constant'', even when we use the Vinogradov notation. We stress that the big-$O$ constant dependencies are always as written so, for example, if $f(x) \ll g(x)$ then the big $O$-constant is absolute.
\end{notation}

==> article/content/negative_integer_case.tex <==
%auto-ignore

\section{Negative integer case}

It is equivalent to count integer solutions to
\begin{align*}
    (x_2x_3x_4)^n + (x_1x_3x_4)^n =
    (x_1x_2x_4)^n + (x_1x_2x_3)^n
\end{align*}
when $n$ is a positive integer. If $p \mid x_1$ is prime, then $p$ divides $x_2$, $x_3$ or $x_4$. Thus we may cancel primes to assume $x_1 = 1$. Let $a_i = \gcd(x_2, x_i)$ and $x_i = a_i y_i$ for $i \in \{3, 4\}$. Then
\begin{align*}
    a_3^na_4^ny_3^ny_4^n(x_2^n + 1) =
    x_2^n(x_4^n + x_3^n).
\end{align*}
Let $x_2 = a_3z_3 = a_4z_4$. Then
\begin{align*}
    a_4^ny_3^ny_4^n(1 + x_2^n) = z_3^n(x_3^n + x_4^n).
\end{align*}
Therefore $y_3 \mid z_3x_4 = a_4z_3y_4$. Since $(y_3, a_4) = (y_3, z_3) = 1$ we must have $y_3 \mid y_4$. By symmetry $y_3 = y_4 = y$, say. Then
\begin{align*}
    a_4^ny^n(1 + x_2^n) = z_3^n(a_3^n + a_4^n).
\end{align*}
We will consider whether $z_3 = 1$ or not.

Suppose that $z_3 = 1$, so that $x_2 = a_3$, and the equation is
\begin{align*}
    a_4^n y^n (1 + a_3^n) = a_3^n + a_4^n.
\end{align*}
Then $a_4 \mid a_3$, say $a_3 = w a_4$. Hence
\begin{align*}
    y^n(1 + a_3^n) = w^n + 1.
\end{align*}


\begin{align*}
    (a_3a_4y)^n(x_2^n + 1) =
    x_2^n(a_3^n + a_4^n)
\end{align*}
Let $x_2 = a_iz_i$ for $i \in \{3, 4\}$. Then
\begin{align*}
    (a_3y)^n(a_4^nz_4^n + 1) = z_4^n(a_3^n + a_4^n).
\end{align*}
Here $(z_4, y) = 1$. Then $z_4 = 1$ or $z_4 \mid a_3$.

In the first case, we have
\begin{align*}
    a_3^ny^n(a_4^n + 1) = a_3^n + a_4^n
\end{align*}
so that $a_3$ divides $a_4$, say $a_4 = ba_3$. Then
\begin{align*}
    y^n(b^na_3^n + 1) = 1 + b^n
\end{align*}
Now the left side is too large except when $y = 1$ and $a_3 = 1$. Hence
\begin{align*}
    x_1 = 1, x_2 = b, x_3 = 1, x_4 = b.
\end{align*}

In the second case, let $a_3 = w_3 z_4$. The equation is
\begin{align*}
    w_3^n y^n (a_4^nz_4^n + 1) = w_3^nz_4^n + a_4^n
\end{align*}
so $w_3 \mid a_4$ as well, say $a_4 = w_3 t_4$. The equation is now
\begin{align*}
    y^n(w_3^n t_4^n z_4^n + 1) = z_4^n + t_4^n.
\end{align*}
Therefore
\begin{align*}
    2\max\{z_4, t_4\}^n \geq
    (yw_3\max\{z_4, t_4\}^2)^n.
\end{align*}
If $n = 1$, then one of $y, w_3$ or $\max\{z_4, t_4\}$ can be equal to $2$, but if $n > 1$ then they are all equal to $1$.

Hence we have proved the following.

\begin{proposition}
    Let $\vec{x} \in \Z_{\geq 1}^4$ with
    \begin{align}
    \label{equation/additive_energy_negative_exponent}
        x_1^{-n} + x_2^{-n} = x_3^{-n} + x_4^{-n},
    \end{align}
    for some positive integer $n$. If $n = 1$, then $\vec{x}$ is an integer multiple of $(1, 2, 2, 1), (1, 2, 1, 2)$ or $(1, 1, 1, 1)$. If $n > 1$, then $\vec{x}$ is an integer multiple of $(1, 1, 1, 1)$. Consequently, the number of solutions $\vec{x} \in [N]^4$ to (\ref{equation/additive_energy_negative_exponent}) is $N$ if $n > 1$ and $2N + O(1)$ if $n = 1$.
\end{proposition}



==> article/content/proofs_of_theorems_on_additive_energy/proof_of_functional_transcendence_lemma.tex <==
%auto-ignore

\begin{proof}
    The proof is by induction on the dimension $n$ of the ambient space. When $n = 1$, the set $X$ consists of a single point, and $f_c(X)$ is contained in a translate of the identity. Assume $n > 1$, and that the result is true when the ambient space has dimension smaller than $n$. 

    Let $d = \dim(X)$ and let $\psi : \R^d \to U \subseteq \exp^{-1}(X)$ be a real-analytic coordinate chart so
    \begin{align*}
        \psi(y_1, \dots, y_d) = (x_1(y_1, \dots, y_d), \dots, x_n(y_1, \dots, y_d))
    \end{align*}
    and the $x_i$ are real-analytic functions on $\R^d$ that we can also regard as elements of $\C[[y_1, \dots, y_d]]$.
    
    We first apply Ax's theorem \cite[Theorem 3]{Ax_on_Schanuel's_conjectures} to the functions $x_1, \dots, x_n$ and $cx_1, \dots, cx_n$. There are two cases to consider. Suppose first that the functions are $\Q$-linearly independent modulo constants, so that the inequality
    \begin{align*}
        \trdeg_{\C}(x_1, \dots, cx_n, \exp(x_1), \dots, \exp(cx_n)) \geq 2n + 
        \rank\bigg(\frac{\partial x_1}{\partial y_1}, \dots, c\frac{\partial x_n}{\partial y_d}\bigg)
    \end{align*}
    holds. Since $\psi$ is a diffeomorphism,
    \begin{align*}
        \rank\bigg(\frac{\partial x_1}{\partial y_1}, \dots, c\frac{\partial x_n}{\partial y_d}\bigg)
        =
        \rank\bigg(\frac{\partial x_i}{\partial y_j}\bigg) = \rank(d\psi) = 
        d.
    \end{align*}
    We also have
    \begin{align*}
        \trdeg_{\C}(\exp(x_1), \dots, \exp(cx_n)) \leq
        \dim(X) + \dim(f_c(X)^{\Zar}).
    \end{align*}
    Therefore $\dim(f_c(X)^{\Zar}) \geq n$, so the Zariski closure of $f_c(X)$ is the coset $\G_m^n$.
    
    We now suppose that the functions are $\Q$-linearly dependent modulo constants in Ax's theorem. By clearing denominators and using the fact that the functions are real-valued, we can assume they are $\Z$-linearly dependent modulo $\R$. Let $r_1, \dots, r_n, s_1, \dots, s_n$ be integers, not all of which are zero, with
    \begin{align*}
        (r_1 + cs_1)x_1 + \dots + (r_n + cs_n)x_n \in \R.
    \end{align*}
    Note that $r_i + cs_i = 0$ if and only if $r_i = s_i = 0$ because $c$ is irrational. In particular, not all of the coefficients $r_i + cs_i$ can vanish, and so we have $\trdeg_{\C}(x_1, \dots, x_n) < n$ \textit{a fortiori}. We can now obtain more information by applying Ax's theorem \cite[Theorem 3]{Ax_on_Schanuel's_conjectures} to the functions $x_1, \dots, x_n$. Case (1) of the theorem implies $\trdeg_{\C}(x_1, \dots, x_n) \geq n$, contrary to what has just been demonstrated. Therefore case (2) occurs, and the functions $x_1, \dots, x_n$ are $\Q$-linearly dependent modulo $\C$; without loss of generality $\Z$-linearly dependent modulo $\R$. If $\vec{a} \in \Z^n$ and $\lambda$ is real with
    \begin{align*}
        a_1x_1 + \dots + a_nx_n = \lambda,
    \end{align*}
    then we can divide $\lambda$ by $\gcd(a_1, \dots, a_n)$ to assume that $\vec{a}$ is a primitive vector. Exponentiating, it follows that the $X$ is contained in a coset $\vec{g}T$, where $\vec{g}$ can be taken to be $(\exp(\lambda/a_1), 1, \dots, 1)$ and $T$ is the $(n - 1)$-dimensional subtorus corresponding to the rank one primitive lattice generated by $\vec{a}$. The conclusion of the lemma can be seen to hold for $X$ if and only if it holds for $\vec{g}^{-1}X$. Thus we can replace the coset $\vec{g}T$ with the torus $T$. Choose an $n \times (n - 1)$ full rank matrix $A$ with integer entries so that the associated monoidal transformation $\phi_A : \G_m^{n - 1} \to \G_m^n$ is a subgroup scheme isomorphism onto $T$.
    
    If $\vec{g} \in \G_m^{n - 1}(\R)$ with $\phi_A(\vec{g}) \in \R_{>0}^n$, write $\vec{g} = \vec{e}\vec{h}$ where $\vec{e} \in \{\pm 1\}^{n - 1}$ and $\vec{h} \in \R_{>0}^{n - 1}$. Then $\phi_A(\vec{e}) \in \R_{>0}^n$ so $\phi_A(\vec{e}) = (1, \dots, 1)$, but then $\vec{e} = (1, \dots, 1)$ since $\phi_A$ is an isomorphism. Therefore $\phi_A^{-1}(\R_{>0}^n) \subseteq \R_{>0}^{n - 1}$ so in particular $\phi_A^{-1}(X) \subseteq \R_{>0}^{n - 1}$. Moreover, $\phi_A^{-1}(X)$ is semi-algebraic since $\phi_A$ is a morphism and connected since $\phi_A$ is an injective open map.
    
    By the inductive hypothesis, the Zariski closure of $f_c(\phi_A^{-1}(X))$ in $\G_m^{n - 1}$ is a coset. Now we have
    \begin{align*}
        \phi_A(f_c(\phi_A^{-1}(X))^{\Zar}) &=
        \phi_A(f_c(\phi_A^{-1}(X)))^{\Zar} \\ &=
        \phi_A(\phi_A^{-1}(f_c(X)))^{\Zar} \\ &=
        f_c(X)^{\Zar}.
    \end{align*}
    Since $\phi_A$ sends cosets to cosets, the Zariski closure of $f_c(X)$ is a coset.
\end{proof}

% \noindent\textbf{Proof of Proposition \ref{proposition/functional_transcendence_proposition}.} The proof is by induction on the dimension $n$ of the ambient space. When $n = 1$, the set $X$ consists of a single point, and $f_c(X)$ is contained in a translate of the identity. Assume $n > 1$, and that the result is true when the ambient space has dimension smaller than $n$. 

% Let $d = \dim(X)$ and let $\psi : \R^d \to U \subseteq \exp^{-1}(X)$ be a real-analytic coordinate chart so
% \begin{align*}
%     \psi(y_1, \dots, y_d) = (x_1(y_1, \dots, y_d), \dots, x_n(y_1, \dots, y_d))
% \end{align*}
% and the $x_i$ are real-analytic functions on $\R^d$ that we can also regard as elements of $\C[[y_1, \dots, y_d]]$.

% We first apply Ax's theorem \cite[Theorem 3]{Ax_on_Schanuel's_conjectures} to the functions $x_1, \dots, x_n$ and $cx_1, \dots, cx_n$. There are two cases to consider. Suppose first that the functions are $\Q$-linearly independent modulo constants, so that the inequality
% \begin{align*}
%     \trdeg_{\C}(x_1, \dots, cx_n, \exp(x_1), \dots, \exp(cx_n)) \geq 2n + 
%     \rank\bigg(\frac{\partial x_1}{\partial y_1}, \dots, c\frac{\partial x_n}{\partial y_d}\bigg)
% \end{align*}
% holds. Since $\psi$ is a diffeomorphism,
% \begin{align*}
%     \rank\bigg(\frac{\partial x_1}{\partial y_1}, \dots, c\frac{\partial x_n}{\partial y_d}\bigg)
%     =
%     \rank\bigg(\frac{\partial x_i}{\partial y_j}\bigg) = \rank(d\psi) = 
%     d.
% \end{align*}
% We also have
% \begin{align*}
%     \trdeg_{\C}(\exp(x_1), \dots, \exp(cx_n)) \leq
%     \dim(X) + \dim(f_c(X)^{\Zar}).
% \end{align*}
% Therefore $\dim(f_c(X)^{\Zar}) \geq n$, so the Zariski closure of $f_c(X)$ is the coset $\G_m^n$.

% We now suppose that the functions are $\Q$-linearly dependent modulo constants in Ax's theorem. By clearing denominators and using the fact that the functions are real-valued, we can assume they are $\Z$-linearly dependent modulo $\R$. Let $r_1, \dots, r_n, s_1, \dots, s_n$ be integers, not all of which are zero, with
% \begin{align*}
%     (r_1 + cs_1)x_1 + \dots + (r_n + cs_n)x_n \in \R.
% \end{align*}
% Note that $r_i + cs_i = 0$ if and only if $r_i = s_i = 0$ because $c$ is irrational. In particular, not all of the coefficients $r_i + cs_i$ can vanish, and so we have $\trdeg_{\C}(x_1, \dots, x_n) < n$ \textit{a fortiori}. We can now obtain more information by applying Ax's theorem \cite[Theorem 3]{Ax_on_Schanuel's_conjectures} to the functions $x_1, \dots, x_n$. Case (1) of the theorem implies $\trdeg_{\C}(x_1, \dots, x_n) \geq n$, contrary to what has just been demonstrated. Therefore case (2) occurs, and the functions $x_1, \dots, x_n$ are $\Q$-linearly dependent modulo $\C$; without loss of generality $\Z$-linearly dependent modulo $\R$. If $\vec{a} \in \Z^n$ and $\lambda$ is real with
% \begin{align*}
%     a_1x_1 + \dots + a_nx_n = \lambda,
% \end{align*}
% then we can divide $\lambda$ by $\gcd(a_1, \dots, a_n)$ to assume that $\vec{a}$ is a primitive vector. Exponentiating, it follows that the $X$ is contained in a coset $\vec{g}T$, where $\vec{g}$ can be taken to be $(\exp(\lambda/a_1), 1, \dots, 1)$ and $T$ is the $(n - 1)$-dimensional subtorus corresponding to the rank one primitive lattice generated by $\vec{a}$. The conclusion of the lemma can be seen to hold for $X$ if and only if it holds for $\vec{g}^{-1}X$. Thus we can replace the coset $\vec{g}T$ with the torus $T$. Choose an $n \times (n - 1)$ full rank matrix $A$ with integer entries so that the associated monoidal transformation $\phi_A : \G_m^{n - 1} \to \G_m^n$ is a subgroup scheme isomorphism onto $T$.

% If $\vec{g} \in \G_m^{n - 1}(\R)$ with $\phi_A(\vec{g}) \in \R_{>0}^n$, write $\vec{g} = \vec{e}\vec{h}$ where $\vec{e} \in \{\pm 1\}^{n - 1}$ and $\vec{h} \in \R_{>0}^{n - 1}$. Then $\phi_A(\vec{e}) \in \R_{>0}^n$ so $\phi_A(\vec{e}) = (1, \dots, 1)$, but then $\vec{e} = (1, \dots, 1)$ since $\phi_A$ is an isomorphism. Therefore $\phi_A^{-1}(\R_{>0}^n) \subseteq \R_{>0}^{n - 1}$ so in particular $\phi_A^{-1}(X) \subseteq \R_{>0}^{n - 1}$. Moreover, $\phi_A^{-1}(X)$ is semi-algebraic since $\phi_A$ is a morphism and connected since $\phi_A$ is an injective open map.

% By the inductive hypothesis, the Zariski closure of $f_c(\phi_A^{-1}(X))$ in $\G_m^{n - 1}$ is a coset. Now we have
% \begin{align*}
%     \phi_A(f_c(\phi_A^{-1}(X))^{\Zar}) &=
%     \phi_A(f_c(\phi_A^{-1}(X)))^{\Zar} \\ &=
%     \phi_A(\phi_A^{-1}(f_c(X)))^{\Zar} \\ &=
%     f_c(X)^{\Zar}.
% \end{align*}
% Since $\phi_A$ sends cosets to cosets, the Zariski closure of $f_c(X)$ is a coset.

% \noindent\textbf{Q.E.D.}

==> article/content/proofs_of_theorems_on_additive_energy/proof_of_theorem_1.tex <==
%auto-ignore

\section{Proof of Theorem \ref{irrational_additive_energy_theorem}}
\label{section/proof_of_additive_energy_bound}

The main term in Theorem \ref{irrational_additive_energy_theorem} comes from the trivial solutions to the equation
\begin{align}
    x_1^c + x_2^c = x_3^c + x_4^c,
    \tag{\ref{additive_energy_equation}}
\end{align}
namely the solutions with $x_1 \in \{x_3, x_4\}$. Henceforth, we let
\begin{align}
        \label{equation/definition_of_B(c, N)}
        B(c, N) =
        \card
        \bigg\{
        \vec{x} \in [N]^4 \; :
        \begin{array}{l}
            x_1^c + x_2^c = x_3^c + x_4^c \\
            x_1 \not \in \{x_3, x_4\} 
        \end{array}
        \bigg\}
\end{align}
denote the number of non-trivial solutions.

Throughout we let $\G_m$ denote the split algebraic torus over $\C$ of dimension one. We often work with $\G_m(\R) = \R^\ast$. A geometrically irreducible algebraic subgroup of $\G_m^n$ is called a subtorus, and a translate of a subtorus by a point of $\G_m^n$ is called a coset. The reader can consult \cite[Chapter 3]{Bombieri--Gubler_heights_in_Diophantine_geometry} for more information about algebraic tori. In particular, we shall assume that the reader is acquainted with the duality between algebraic subgroups of $\G_m^n$ and subgroups in $\Z^n$.

The following description of the abelian group $\Hom_{\textbf{AlgGrp}}(\G_m^r, \G_m^s)$ will be crucial for the argument. If $A = (a_{ij})$ is an $r \times s$ matrix with integer entries, we can define a morphism of algebraic groups
\begin{align*}
    \phi_A : \G_m^r &\to \G_m^s \\
    (x_1, \dots, x_r) &\mapsto
    (x_1^{a_{11}} \dots x_r^{a_{r1}}, \dots,
    x_1^{a_{1s}} \dots x_r^{a_{rs}}).
\end{align*}
In \cite[Proposition 3.2.17]{Bombieri--Gubler_heights_in_Diophantine_geometry}, it is proved that the map sending $A$ to $\phi_A$ is an isomorphism of the abelian groups $M_{r, s}(\Z)$ and $\Hom_{\textbf{AlgGrp}}(\G_m^r, \G_m^s)$.

The kernel of $\phi_A$ is the subgroup associated to the lattice $\Lambda \subseteq \Z^r$ spanned by the columns of $A$. If $r \leq s$ and the rank of $A$ is $r$, then the kernel of $\phi_A$ is zero-dimensional, and its cardinality is the index of $\Lambda$ in $\Lambda_{\R} \cap \Z^r$ \cite[Proposition 3.2.7]{Bombieri--Gubler_heights_in_Diophantine_geometry}. In particular, $\phi_A$ is injective if and only if $r \leq s$, $A$ is of rank $r$ and $\Lambda$ is a primitive lattice.

%%% Perhaps it would be good to replace n,m by r,s? Also, I do not  understand your argument about injectivity. The map $(x,y) --> x/y$ has rank 1 and kernel $\{(x,x)\}$. Do you mean to say that $m \geq n$? But then  $x --> x^2$ has non-trivial kernel and full rank. Do you mean  the map is injective when restricted to the orthan or do you rather want $\varphi$ to be primitve?     

%%removed the statement about injectivity, because it isn't used later.

\begin{lemma}
\label{lemma/preimage_of_orthant_under_monoidal_transformation}
    Let $\phi_A : \G_m^r \to \G_m^s$ be the morphism associated to an $r \times s$ matrix $A$ with integer entries. Suppose $\phi_A$ is injective. Then 
    \begin{align*}
        \phi_A^{-1}(\R_{> 0}^s) \cap \G_m^r(\R) \subseteq \R_{> 0}^r.
    \end{align*}
\end{lemma}
\begin{proof}
    Suppose $\vec{g} \in \G_m^r(\R)$ and $\phi_A(\vec{g}) \in \R_{> 0}^m$. We can write $\vec{g} = \vec{s} \vec{h}$ where $\vec{s} \in \{-1, 1\}^r$ is the signed part of $\vec{g}$ and $\vec{h} \in \R_{> 0}^r$. Since the coordinate functions of $\phi_A$ are monomials, we have $\phi_A(\vec{s}) \in \{-1, 1\}^s$ and $\phi_A(\vec{h}) \in \R_{> 0}^s$. The latter implies that $\phi_A(\vec{s}) \in \R_{> 0}^s$, and so $\phi_A(\vec{s}) = (1, \dots, 1)$ is the identity. Since $\phi_A$ is injective, $\vec{s} = (1, \dots, 1)$. Thus $\vec{g} \in \R_{> 0}^r$.
\end{proof}

If $X \subseteq \G_m^n(\R)$, we let $X^{\Zar}$ denote the Zariski closure of $X$ in $\G_m^n(\C)$, which is a subscheme of $\G_m^n$. We will only be taking Zariski closures inside $\G_m^n$ and so this notation should not cause confusion.

Recall that a subset $X$ of $\R^n$ is called semi-algebraic if it is a Boolean combination of sets of the form $\{\vec{x} \in \R^n : f(\vec{x}) > 0\}$ or $\{\vec{x} \in \R^n : f(\vec{x}) = 0\}$, where $f$ is a polynomial with real coefficients. The semi-algebraic sets enjoy the favourable feature of remaining semi-algebraic after coordinate projections, as proved by Tarski and Seidenberg. We say that a semi-algebraic set is irreducible if its Zariski closure is irreducible, and we say that a semi-algebraic set is smooth if it consists of only smooth points of its Zariski closure.

In the proof of Theorem \ref{irrational_additive_energy_theorem}, we shall be working with the structure $\R_{\exp}$. Let us just say that a structure prescribes a collection of subsets of each Euclidean space $\R^n$, that are said to be the definable sets in that structure. A subset $X$ of $\R^n$ is definable in $\R_{\exp}$ if and only if $X$ can be obtained via Boolean operations, products and coordinate projections of either semi-algebraic sets, or the graph in $\R^2$ of the real exponential function. A theorem of Wilkie \cite{Wilkie_model_completeness_results_for_expansions_of_the_ordered_field_of_real_numbers_by_restricted_Pfaffian_functions_and_the_exponential_functions} implies that the structure $\R_{\exp}$ is o-minimal, i.e., the definable subsets of $\R$ are finite unions of points and intervals. We refer the reader to \cite{Van_den_Dries_tame_topology_and_o-minimal_structures} for more information about semi-algebraic sets and o-minimal structures.

\subsection{Functional transcendence}

The following proposition is where we need to assume that $c$ is irrational for our argument. The proposition is not true if $c$ is rational. For example, if $c = a/q$ is rational and $Z$ is the algebraic curve $x^a + y^a = 1$, then $f_c(Z)$ lies inside the algebraic curve $x^q + y^q = 1$, which is not a translate of an algebraic subgroup of $\G_m^2$.

\begin{proposition}
    \label{proposition/functional_transcendence_proposition}
    Let $X$ be a semi-algebraic set in $\R_{>0}^n$. Moreover, let $c$ be a real irrational number and let $f_c$ denote the map
    \begin{align*}
        f_c : \R^n_{> 0} &\to \R^n_{> 0} \\
        (x_1, \dots, x_n) &\mapsto (x_1^c, \dots, x_n^c).
    \end{align*}
    The Zariski closure of $f_c(X)$ in $\G_m^n$ is a finite union of cosets.
\end{proposition}
\begin{proof}
    First, we can stratify the semi-algebraic set $X$ into finitely many semi-algebraic subsets that are smooth and connected. If the statement of the lemma holds for each piece, then it holds for $X$. Thus we can assume that $X$ is smooth and connected. In particular, it is a real-analytic manifold.

    The proof is by induction on the dimension $n$ of the ambient $\G_m^n$. When $n = 1$, the set $X$ consists of a single point, and $f_c(X)$ is contained in a translate of the identity. Assume $n > 1$, and that the result is true when the ambient space has dimension smaller than $n$. 

    Let $d = \dim(X)$ and let $\psi : \R^d \to U \subseteq \exp^{-1}(X)$ be a real-analytic chart of the real logarithm $\exp^{-1}(X)$ of $X$. Thus there are real-analytic functions $u_1, \dots, u_n : \R^d \to \R$ such that
    \begin{align*}
        \psi(y_1, \dots, y_d) = (u_1(y_1, \dots, y_d), \dots, u_n(y_1, \dots, y_d))
    \end{align*}
    parameterises the chart $U$ of $X$. We can regard each $u_i$ as an element of the ring $\C[[y_1, \dots, y_d]]$.
    
    We first apply Ax's theorem \cite[Theorem 3]{Ax_on_Schanuel's_conjectures} to the functions $u_1, \dots, u_n$ and $cu_1, \dots, cu_n$. There are two cases to consider. Suppose first that these functions are $\Q$-linearly independent modulo $\C$, so that by Ax's theorem the transcendence degree of the $4n$ functions
    \begin{align*}
        u_1, \dots, u_n, cu_1, \dots, cu_n, \exp(u_1), \dots, \exp(u_n),
        \exp(cu_1), \dots, \exp(cu_n)
    \end{align*}
    is at least
    \begin{align*}
        2n + \rank\bigg(
        \frac{\partial u_i}{\partial y_j} \; \bigg\vert \;
        c\frac{\partial u_i}{\partial y_j}
        \bigg)_{\substack{i \in [n] \\ j \in [d]}} =
        2n + \rank\bigg(
        \frac{\partial u_i}{\partial y_j}
        \bigg)_{\substack{i \in [n] \\ j \in [d]}}.
    \end{align*}
    Since $\psi$ is a diffeomorphism, this latter expression is equal to $2n + d$. Note that, by construction, the functions $\exp(u_1), \dots, \exp(u_n)$ parameterise the chart $\exp(U)$ of $X$ and the functions $\exp(cu_1), \dots, \exp(cu_n)$ parameterise the chart $f_c(\exp(U))$ of $f_c(X)$. In particular, since $\exp(U)$ is semi-algebraic,
    \begin{align*}
        \trdeg_{\C}(\exp(u_1), \dots, \exp(u_n)) = \dim(\exp(U)) = \dim(X).
    \end{align*}
    The same equalities for $f_c(\exp(U))$ and $f_c(X)^{\Zar}$ shows that
    \begin{align*}
        \trdeg_{\C}(\exp(u_1), \dots, \exp(u_n), \exp(cu_1), \dots, \exp(cu_n)) \leq
        d + \dim(f_c(X)^{\Zar}).
    \end{align*}
    Therefore 
    \begin{align*}
        \dim(f_c(X)^{\Zar}) &\geq
        \trdeg_{\C}(\exp(u_1), \dots, \exp(u_n), \exp(cu_1), \dots, \exp(cu_n)) - d
        \\ &\geq
        2n + d - \trdeg_{\C}(u_1, \dots, u_n) - d
        \\ &\geq n.
    \end{align*}
    Since $\G_m^n$ is irreducible and $f_c(X)^{\Zar}$ is closed, the Zariski closure of $f_c(X)$ is the coset $\G_m^n$.
    
    We now suppose that the functions $u_1, \dots, u_n, cu_1, \dots, cu_n$ are $\Q$-linearly dependent modulo $\C$ in Ax's theorem. By clearing denominators and using the fact that the functions are real-valued, we can assume they are $\Z$-linearly dependent modulo $\R$. Let $r_1, \dots, r_n, s_1, \dots, s_n$ be integers, not all of which are zero, with
    \begin{align*}
        (r_1 + cs_1)u_1 + \dots + (r_n + cs_n)u_n \in \R.
    \end{align*}
    Note that $r_i + cs_i = 0$ if and only if $r_i = s_i = 0$ because $c$ is irrational. In particular, not all of the coefficients $r_i + cs_i$ can vanish, and so we have $\trdeg_{\C}(u_1, \dots, u_n) < n$. We can now obtain more information by applying Ax's theorem to the functions $u_1, \dots, u_n$. The $\Q$-linearly independent modulo $\C$ case of the theorem implies $\trdeg_{\C}(u_1, \dots, u_n) \geq n$, contrary to what has just been demonstrated. Therefore the functions $u_1, \dots, u_n$ are $\Q$-linearly dependent modulo $\C$; without loss of generality $\Z$-linearly dependent modulo $\R$. If $\vec{a} = (a_1, \dots, a_n) \in \Z^n$ and $\lambda$ is real with
    \begin{align*}
        a_1u_1 + \dots + a_nu_n = \lambda,
    \end{align*}
    then we can divide $\lambda$ by $\gcd(a_1, \dots, a_n)$ to assume that $\vec{a}$ is a primitive vector. Exponentiating, it follows that $\exp(U)$ is contained in a coset $\vec{g}T$, where $\vec{g}$ can be taken to be $(\exp(\lambda/a_1), 1, \dots, 1)$ and $T$ is the $(n - 1)$-dimensional subtorus corresponding to the rank one primitive lattice generated by $\vec{a}$.(  See \cite[Section 3.2.6]{Bombieri--Gubler_heights_in_Diophantine_geometry}. ) Since $X$ is irreducible, the Zariski closure of $\exp(U)$ contains $X$, and is contained in $\vec{g}T$.

    The conclusion of the lemma can be seen to hold for $X$ if and only if it holds for $\vec{g}^{-1}X$. Thus we can replace the coset $\vec{g}T$ with the torus $T$. Choose an $n \times (n - 1)$ full rank matrix $A$ with integer entries so that the associated morphism of algebraic groups $\phi_A : \G_m^{n - 1} \to \G_m^n$ is an isomorphism onto $T$.

    To apply the inductive hypothesis to $\phi_A^{-1}(X)$ lying inside $\G_m^{n - 1}(\R)$, we need to show that the hypotheses of the proposition are satisfied for $\phi_A^{-1}(X)$. By Lemma \ref{lemma/preimage_of_orthant_under_monoidal_transformation} we have $\phi^{-1}_A(X) \subseteq \R_{> 0}^{n - 1}$. Moreover, $\phi_A^{-1}(X)$ is semi-algebraic since $\phi_A$ is a morphism and connected since $\phi_A$ is an injective open map.
    
    By the inductive hypothesis, the Zariski closure of $f_c(\phi_A^{-1}(X))$ in $\G_m^{n - 1}$ is a finite union of cosets. Now we have
    \begin{align*}
        \phi_A(f_c(\phi_A^{-1}(X))^{\Zar}) &=
        \phi_A(f_c(\phi_A^{-1}(X)))^{\Zar} \\ &=
        \phi_A(\phi_A^{-1}(f_c(X)))^{\Zar} \\ &=
        f_c(X)^{\Zar},
    \end{align*}
    where we have used the fact that $f_c$ commutes with any morphism of algebraic groups $\phi_A$. Since $\phi_A$ sends cosets to cosets \cite[Proposition 3.2.18]{Bombieri--Gubler_heights_in_Diophantine_geometry}, the Zariski closure of $f_c(X)$ is a finite union of cosets.
\end{proof}

\subsection{O-minimal point counting}

We now describe heights and the o-minimal point counting results that will be used in the proof of Theorem \ref{irrational_additive_energy_theorem}. If a rational number can be written as $a/q$ where $a$ and $q > 0$ are coprime integers, then we define the height $H(a/q) = \max(\abs{a}, q)$. The height of $\vec{x} \in \Q^n$ is $H(\vec{x}) = \max_i \{H(x_i)\}$. If $X$ is a subset of $\R^n$ and $T > 0$, we let
\begin{align*}
    X(\Q, T) = \{\vec{x} \in X \cap \Q^n : H(\vec{x}) \leq T\}.
\end{align*}
We also define the algebraic part of $X$
\begin{align*}
    X^{\alg} = \bigcup_{\substack{Z \subseteq X \\ \\ \textrm{$Z$ semi-algebraic} \\ \\ \dim(Z) > 0}}
    Z
\end{align*}
and the transcendental part $X^{\trans} = X \setminus X^{\alg}$. Thus the points of $X^{\alg}$ are exactly the points of $X$ that lie on semi-algebraic curves.

\begin{theorem}
    \cite[Theorem 1.8]{Pila--Wilkie_the_rational_points_on_a_definable_set}
    Let $X$ be a subset of $\R^n$ definable in an o-minimal structure. Then
    \begin{align*}
        \card X^\trans(\Q, N) \ll_\eps N^\eps
    \end{align*}
    for every $\eps > 0$.
\end{theorem}

The estimate provided by the Pila--Wilkie theorem is already good enough to prove $B(c, N) \ll_{\eps} N^{1 + \eps}$ together with Lemma \ref{lemma/algebraic_part_of_Y}, however we will be able to prove $B(c, N) \ll N(\log{N})^\alpha$ for some $\alpha > 0$ using the following theorem, which was already conjectured in \cite[Conjecture 1.11]{Pila--Wilkie_the_rational_points_on_a_definable_set}. Here we use the version of the theorem for definable families, which allows us to achieve uniformity in the exponent $c$. 

% To achieve the same quality of upper bound without effective constants, we could have employed an earlier result \cite[Theorem 1.5]{Jones--Thomas_the_density_of_algebraic_points_on_certain_Pfaffian_surfaces} of Jones--Thomas.

\begin{theorem}
    \label{theorem/Binyamini--Novikov--Zak_result}
    \cite[Equation (6)]{Binyamini--Novikov--Zak_Wilkie's_conjecture_for_Pfaffian_structures}
    Let $X \to \Lambda$ be an $\R_{\exp}$-definable family. There exists an effectively computable $\alpha > 0$ such that for any $\lambda \in \Lambda$
    \begin{align*}
        \card{X^{\trans}_\lambda (\Q, T)} \ll_X (\log{T})^\alpha.
    \end{align*}
\end{theorem}

In particular, the big-O constant depends on the definable family, but not on the parameter $\lambda$.

\subsection{Proof of Theorem \ref{irrational_additive_energy_theorem}}
\label{proof_of_theorem_A/proof_of_theorem_A}

We consider the $\R_{\exp}$-definable set
\begin{align*}
    X = \{(c, \vec{x}) \in \R \times \R_{>0}^4 : x_1^c + x_2^c = x_3^c + x_4^c\},
\end{align*}
which becomes a definable family when equipped with the projection $X \to \R$ onto the first coordinate. We also define
\begin{align*}
    X^{\textrm{nt}} = \{(c, \vec{x}) \in X : x_1 \in \{x_3, x_4\}\},
\end{align*}
the $\R_{\exp}$-definable subset of $X$ containing only the non-trivial solutions of (\ref{additive_energy_equation}). Here it is clear that these sets are definable in $\R_{\exp}$, because $x^c = \exp(c\log{x})$.

In this situation, one has the crude bound
\begin{align*}
    B(c, N) \ll \card X^{\textrm{nt}}_c(\Q, N),
\end{align*}
and a naive approach to proving Theorem \ref{irrational_additive_energy_theorem} would involve showing that $X^{\textrm{nt}}$ and $X^{\trans}$ coincide, and then using Theorem \ref{theorem/Binyamini--Novikov--Zak_result}.

Unfortunately, this simply does not work because $X^{\alg} = X$ in this case. To circumvent this issue, we consider the dehomogenised families
\begin{align*}
    Y &= \{(c, \vec{x}) \in \R \times \R_{>0}^3 : 1 + x_1^c = x_2^c + x_3^c\},
    \\
    Y^{\textrm{nt}} &=
    \{(c, \vec{x}) \in Y : x_1 \not \in \{x_2, x_3\}\},
\end{align*}
which are still definable in $\R_{\exp}$. We think of $Y$ as a slice of $X$ under the projection onto the first coordinate. The issue is essentially that some points of $X$ lie on semi-algebraic curves that are horizontal with respect to the projection. Such semi-algebraic curves intersect the dehomogenised slice $Y$ in a zero-dimensional semi-algebraic set, which does not contribute to the algebraic part of $Y$.

It now follows that
\begin{align}
\label{bound_proving_theorem_A}
    B(c, N)
    \ll
    \card X^{\textrm{nt}}_c(\Q, N) \ll
    N \card Y^{\textrm{nt}}_c(\Q, N),
\end{align}
and we must show that $Y^{\textrm{nt}} = Y^{\trans}$ in order to prove Theorem \ref{irrational_additive_energy_theorem}.

\begin{lemma}
\label{lemma/algebraic_part_of_Y}
    It holds that $Y^{\textrm{nt}} = Y^{\trans}$, i.e.,
    \begin{align*}
        Y^{\alg} = \{(c, \vec{x}) \in \R \times \R^3_{>0} : x_1 \in \{x_2, x_3\}\}.
    \end{align*}
\end{lemma}
\begin{proof}
    Let $Z$ be a connected, semi-algebraic curve in $Y$. By Proposition \ref{proposition/functional_transcendence_proposition}, the Zariski closure $W$ of $f_c(Z)$ in $\G_m^3$ is a translate of an algebraic subgroup. On the other hand, it is contained in the hyperplane $H$ defined by $1 + x_1 = x_2 + x_3$. Since this hyperplane is not a translate of an algebraic subgroup, $W$ must be a curve. By \cite[Proposition 3.2.17]{Bombieri--Gubler_heights_in_Diophantine_geometry}, we can choose an isomorphism
    \begin{align*}
        \G_m &\to W \\
        z &\mapsto (\alpha_1 z^{a_1} ,
        \alpha_2 z^{a_2} ,
        \alpha_3 z^{a_3}
        ),
    \end{align*}
    where $(\alpha_1, \alpha_2, \alpha_3) \in \R_{>0}^3$ and $(a_1, a_2, a_3) \in \Z^3$. The image lies in $H$, and so we have the equation
    \begin{align*}
        1 + 
        \alpha_1 z^{a_1}  =
        \alpha_2 z^{a_2}  +
        \alpha_3 z^{a_3}
    \end{align*}
    for all $z \in \R^\times$. Now $a_2 = 0$ or $a_3 = 0$ (we cannot just have $a_1 = 0$, because then $\alpha_1 = -1$). If $a_2 = 0$, then we must have $a_1 = a_3$. Then $\alpha_2 = 1$ and $\alpha_1 = \alpha_3$. It follows that $W$ is the line $x_1 = x_3$ and $x_2 = 1$. Hence $Z$ is contained in this line too. Taking $a_3 = 0$ leads to the other option $x_1 = x_2$ and $x_3 = 1$.
\end{proof}

Lemma \ref{lemma/algebraic_part_of_Y} and Theorem \ref{theorem/Binyamini--Novikov--Zak_result} can now be combined to show
\begin{align*}
    B(c, N) \ll N \card Y_c^{\trans}(\Q, N)
    \ll N(\log{N})^\alpha.
\end{align*}
Since the set $Y$ is existentially definable, the big-O constant in \cite{Binyamini--Novikov--Zak_Wilkie's_conjecture_for_Pfaffian_structures} is effective. We thank Gareth Jones for this observation. This concludes the proof of Theorem \ref{irrational_additive_energy_theorem}.

==> article/content/rational_case.tex <==
%auto-ignore

\section{Rational case}

\begin{lemma}
\label{lemma/sporadic_primitive_solutions_must_be_powers}
    Let $c = a/q$ with $a$ and $q > 1$ coprime integers and let $\vec{x}$ be a primitive sporadic solution. Then each coordinate of $\vec{x}$ is a $q$-th power.
\end{lemma}
\begin{proof}
    This follows from \cite[Proposition 4.1]{Carr--O'Sullivan_on_the_linear_independence_of_roots}.
\end{proof}

\begin{theorem}
    Let $c = a/q$ with $a$ and $q > 0$ coprime integers. Then
    \begin{align*}
        \card\{\vec{x} \in [n]^4 : x_1^c + x_2^c = x_3^c + x_4^c\} = 2n^2 + O_{c, \eps}(n).
    \end{align*}
\end{theorem}
\begin{proof}
    We first suppose $a > 0$. By Lemma \ref{lemma/sporadic_primitive_solutions_must_be_powers} and \cite[Corollary 0.7]{Salberger_counting_rational_points_on_projective_varieties}
    \begin{align*}
        \sum_{\substack{\vec{x} \in [n]^4 \\ \textrm{$\vec{x}$ sporadic}}} 1 &=
        \sum_{d \leq n}
        \sum_{\substack{\vec{x} \in [n^{1/q}d^{-1/q}]^4 \\ \textrm{$\vec{x}$ primitive, sporadic}}} 1 \\ &\ll_{a, \eps}
        \sum_{d \leq n} (n^{1/q}d^{-1/q})^{3/a^{1/2} + \eps} \\ &\ll_{a, \eps}
        n^{3/(a^{1/2}q) + \eps} \sum_{d \leq n} d^{-3/(a^{1/2}q) + \eps} \\
        &\ll_{a, \eps}
        n^{3/(a^{1/2}q) + \eps} + n.
    \end{align*}
\end{proof}


==> article/content/upgrading_the_result.tex <==
\section{Upgrading result}

\subsection{More general sets}

Let $A$ be a set of positive rational numbers. By multiplying by a common denominator, we get a set of integers and don't change the size of the sumset.

Hence suppose $A \subseteq \Z$ and $|A + A| \leq K|A|$. By Freiman's theorem $A$ is contained in a proper generalised arithmetic progression $P$ of dimension $d(K) \ll K^4\log(K + 2)$ and size at most $|A|\exp(d(K))$. Hence there are $L_1, \dots, L_d$ with
\begin{align*}
    A \subseteq n_0 + n_1 [L_1] + \dots + n_d [L_d]
\end{align*}
for some integers $n_0, \dots, n_d$. Since $P$ is proper, the sums are distinct and $|P| = L_1 \dots L_d$. 

We need to count points on the surface lying in $P$.

(we can apply this in $\R$ since the subgroup must be finite).

Should get something like $(L_1 \dots L_d)^{1 + \eps} \ll |A|^{1 + \eps}\exp((1 + \eps)d(K))$ perhaps. We just need
\begin{align*}
    \exp((1 + \eps)d(K)) \ll |A|^{2 - \eps}.
\end{align*}
Hence
\begin{align*}
    d(K) \ll 2\log|A|.
\end{align*}
Using the original bounds we only get the sumset result for $K \ll (\log|A|)^4$. However results of Croot and Sisask give something like $K = |A|^{1/3}$.

\subsection{Approximate energy}

Let $Z$ be the set
\begin{align*}
    \{\vec{x} \in \R^3_{>0} : |1 + x_1^c - x_2^c - x_3^c| < 1\},
\end{align*}
which is definable in $\R_{\exp}$.

We consider the shifted, dehomogenised energy set
\begin{align*}
    Z_\delta : 1 + x_1^c - x_2^c - x_3^c = \delta \neq 0.
\end{align*}
If $X$ is a semi-algebraic curve in $Z_\delta$ then $f_c(X)$ lies in $1 + x_1 - x_2 - x_3 = \delta$. We can run the same argument to show that $\delta = 0$. Hence there is no algebraic part in the shifted set.

If the approximate energy contains a non-diagonal semi-algebraic set, then it is the image of some function $(x_1(\delta), x_2(\delta), x_3(\delta))$. the $x_i$ are analytic functions of $\delta$ satisfying
\begin{align*}
    1 + x_1(\delta)^c - x_2(\delta)^c - x_3(\delta)^c = \delta
\end{align*}
for all $\delta$ in an interval.

Suppose $q = (q_1, q_2, q_3)$ approximates a real point $(x_1, x_2, x_3)$ on the dehomogenised energy surface with $|q_i - x_i| < \eps$, say. We know that
\begin{align*}
    q_i^c - x_i^c = c(q_i - x_i) \xi_i^{c - 1}
\end{align*}
for some $\xi_i$ lying between $q_i$ and $x_i$. We think of $c$ as small so that
\begin{align*}
    |q_i^c - x_i^c| \leq
    |c| \eps \min(|q_i|, x_i)^{c - 1}
\end{align*}

Then
\begin{align*}
    |1 + q_1^c - q_2^c - q_3^c| 
    &\leq
    |1 + x_1^c - x_2^c - x_3^c| +
    |q_1^c - x_1^c| + |q_2^c - x_2^c| + |q_3^c - x_3^c|
    \\
    &\leq
    3|c|\eps N^{1 - c}.
\end{align*}
Just need to make $\eps$ small enough that this is $< 1$.

This prove that there are few points on the approximate energy surface away from the algebraic part.

Since we are approximating the surface, we only need to understand rational points in thickenings of the diagonal lines. Note: to apply Habegger's definable diophantine approximation result, we need a polynomially bounded structure. For this we use the Pfaffian structure with chain $x^c, 1/x$.

This would be one approach towards getting an estimate for the exponential sums.

We also have
\begin{align*}
    \int_0^1 \left|
    \sum_{n \leq N} e(\theta n^c)
    \right|^2
    \; d\theta =
    \sum_{n_1, n_2 \leq N}
    \int_0^1
    e(\theta(n_1^c - n_2^c)) \; d\theta =
    N +
    \sum_{n_1, n_2 \leq N} \frac{e(n_1^c - n_2^c) - 1}{n_1^c - n_2^c}.
\end{align*}
Should be possible to show other thing has size $N$.

\subsection{Better solution forbidding $c$ region}

Expanding each $n_i^c = \exp((\log{n_i})c)$ using the Taylor series for the exponential function gives
\begin{align*}
    n_1^c + n_2^c - n_3^c - n_4^c =
    c\log\left(\frac{n_1n_2}{n_3n_4}\right)
    + \sum_{i \geq 2} \frac{c^i}{i!} \left(
    (\log{n_1})^i +
    (\log{n_2})^i - (\log{n_3})^i - (\log{n_4})^i
    \right)
\end{align*}
The remainder term is at most
\begin{align*}
    4\sum_{i \geq 2} \frac{c^i}{i!} (\log{N})^i \leq
    4 c^2 (\log{N})^2 N^c.
\end{align*}
If $(n_1, n_2, n_3, n_4)$ is a solution to the equation then
\begin{align*}
    \log\left(\frac{n_3n_4}{n_1n_2}\right)
    \leq 4c(\log{N})^2 N^c.
\end{align*}
By the mean value theorem
\begin{align*}
    \left|
    \log\left(
    \frac{n_3n_4}{n_1n_2}
    \right)
    \right|
    \geq \frac{|n_1n_2 - n_3n_4|}{N^2}.
\end{align*}
It follows that if $c < c_0(N)$, where $c_0(N)$ satisfies
\begin{align*}
    4N^2 (\log{N}) (c_0(N)\log{N})\exp(c_0(N) \log{N}) = 1,
\end{align*}
then $n_1 n_2 = n_3 n_4$.

\begin{proposition}
    Let $n_1, n_2, n_3, n_4$ be positive integers satisfying the equations
    \begin{align*}
        n_1 n_2 &= n_3 n_4, \\
        n_1^c + n_2^c &= n_3^c + n_4^c
    \end{align*}
    for a non-zero real number $c$. Then $n_1 = n_3$ or $n_1 = n_4$.
\end{proposition}
\begin{proof}
    Let $d = \gcd(n_1, n_3)$ and write $n_i = a_i d$ for $i \in \{1, 3\}$. Then $a_1 n_2 = a_3 n_4$ and $\gcd(a_1, a_3) = 1$, so $a_1 \mid n_4$ and $a_3 \mid n_2$. Let $n_4 = a_1 b_4$ and $n_2 = a_3 b_2$. Then $a_1 a_3 b_2 = a_1 a_3 b_4$ so $b_2 = b_4 = b$, say. Thus the solutions of $n_1 n_2 = n_3 n_4$ are parameterised by
    \begin{align*}
        (n_1, n_2, n_3, n_4) =
        (a_1 d, a_3 b, a_3 d, a_1 b)
    \end{align*}
    for $a_1, a_3, b, d$ integers with $\gcd(a_1, a_3) = 1$. Thus
    \begin{align*}
        n_1^c + n_2^c - n_3^c - n_4^c = 
        a_1^c d^c + a_3^c b^c - a_3^c d^c - a_1^c b^c =
        (a_1^c - a_3^c)(d^c - b^c) = 0.
    \end{align*}
    It follows that $a_1 = a_3$ or $d = b$. In the first case, $n_1 = n_3$ and in the second case $n_1 = n_4$.
\end{proof}

This proves the following.

\begin{proposition}
    If $c < c_0(N)$ then the equation $n_1^c + n_2^c = n_3^c + n_4^c$ has no off-diagonal solutions in $\{1, \dots, N\}$.
\end{proposition}

It suffices to estimate $c_0(N)$. Note that
\begin{align*}
    c_0(N) \log{N} = W\left(\frac{1}{4N^2 (\log{N})}\right)
\end{align*}
where $W$ is the principal branch of the Lambert $W$-function.

\begin{lemma}
    Let $0 < x \leq \eps/ (e(1 + \eps))$. Then
    \begin{align*}
        (1 - \eps)x \leq W(x) \leq x.
    \end{align*}
\end{lemma}
\begin{proof}
    The upper bound follows easily from the fact $W(x) > 0$ so that $W(x) \leq W(x) \exp(W(x)) = x$.
    
    On the interval $(0, e^{-1})$, the Lambert $W$-function admits a Taylor series expansion
    \begin{align*}
        W(x) = \sum_{n \geq 1} \frac{(-n)^{n - 1}}{n!}x^n
        = x(1 - \sum_{n \geq 1} \frac{(-1)^{n - 1} (n + 1)^{n}}{(n + 1)!} x^n).
    \end{align*}
    There is the basic bound
    \begin{align*}
        \frac{(n + 1)^n}{(n + 1)!} \leq e^n.
    \end{align*}
    It follows that
    \begin{align*}
        \left|
        \sum_{n \geq 1}
        \frac{(-1)^{n - 1}(n + 1)^n}{(n + 1)!}x^n
        \right|
        \leq \sum_{n \geq 1} (ex)^n = \frac{ex}{1 - ex}.
    \end{align*}
    If $ex \leq \eps/(1 + \eps)$ then
    \begin{align*}
        \frac{ex}{1 - ex} \leq \eps
    \end{align*}
    so
    \begin{align*}
        W(x) \geq (1 - \eps)x,
    \end{align*}
    as claimed.
\end{proof}

It follows that if
\begin{align*}
    \frac{1}{4N^2(\log{N})} \leq \frac{\eps}{e(1 + \eps)}
\end{align*}
then
\begin{align*}
    c_0(N) \log{N} \geq \frac{1 - \eps}{4N^2(\log{N})}.
\end{align*}

\begin{align*}
    \frac{4}{e}N^2 \log{N} \geq 1 + \frac{1}{\eps}.
\end{align*}

It we take $N \geq 2$ then we can take $\eps = 1/3$. This gives
\begin{align*}
    c_0(N) \geq \frac{1}{6N^2(\log{N})^2}.
\end{align*}

\begin{theorem}
    Suppose
    \begin{align*}
        0 < c < \frac{1}{6N^2(\log{N})^2}.
    \end{align*}
    Then the equation
    \begin{align*}
        n_1^c + n_2^c = n_3^c + n_4^c
    \end{align*}
    has only diagonal solutions in $\{1, \dots, N\}$.
\end{theorem}

Let $A = \{n^c : n \leq N\}$. Then every non-zero element of the difference set $A - A$ is represented in exactly one way. Indeed if $a_1 - a_3 = a_4 - a_2$ then $a_1 = a_3$ so we represent zero and if $a_1 = a_4$, then we are considering the same represntation. It follows that
\begin{align*}
    |A|^2 = (|A - A| - 1) + |A|
\end{align*}
so  $|A - A| = |A|^2 - |A| + 1$.

Forms a perfect difference set.

For the sumsets, if $a_1 + a_2 = a_3 + a_4$ are two representations of the same sumset element then $a_1 = a_3$ or $a_1 = a_4$. Thus every pair $(a_1, a_2)$ either has $a_1 = a_2$ or represents an element of the sumset twice
\begin{align*}
    |A|^2 = |A| + 2(|A + A| - |A|).
\end{align*}
It follows that the sumset and product set are as large as possible and the additive energy is as small as possible.

\subsection{Forbidden close solutions}

We now assume that $n_i \in [N, 2N]$ so that the remainder term is
\begin{align*}
    2\sum_{i \geq 2} \frac{c^i}{i!}\left(
    (\log{2N})^i
    - (\log{N})^i
    \right).
\end{align*}
We have
\begin{align*}
    x^i - y^i = (x - y) i z^{i - 1}
\end{align*}
where $z$ lies between $x$ and $y$. Hence
\begin{align*}
    (\log{2N})^i - (\log{N})^i = (\log{2}) i (\log{2N})^{i - 1}.
\end{align*}

By the mean value theorem
\begin{align*}
    (\log{2N})^i - (\log{N})^i = 
    \frac{i(\log{\xi})^{i - 1}}{\xi}N
\end{align*}
for some $\xi \in [N, 2N]$. There are three cases to consider: first if $i$ is small compared to $N$, then if the global maximum of the function lies inside $[N, 2N]$, finally the case when $i$ is large compared to $N$.

\subsection{A saving before o-minimal counting}

Suppose $(n_1, n_2, n_3, n_4)$ is a solution with all $n_i$ in $[N^{1 - \delta}, N]$.

Then
\begin{align*}
    c\log\left(
    \frac{n_3n_4}{n_1n_2}
    \right)
    &\leq
    2\sum_{i \geq 2} 
    \frac{c^i}{i!}
    \left(
    (\log{N})^i - (\log{N^{1 - \delta}})^i
    \right)
    \\ &<
    2\sum_{i \geq 2}
    \frac{c^i}{i!}
    \left(
    \log{N} -
    \log(N^{1 - \delta})
    \right)
    i (\log{N})^{i - 1}
    \\ &=
    2\delta \sum_{i \geq 2} \frac{c^i(\log{N})^i}{(i - 1)!}
    \\ &=
    2\delta c (\log{N})
    (N^c - 1).
\end{align*}
Hence
\begin{align*}
    |n_1 n_2 - n_3 n_4| <
    2\delta N^2 (\log{N}) (N^c - 1).
\end{align*}
This shows with the previous proposition that if
\begin{align*}
    \delta(N, c) \leq \frac{1}{2N^2(\log{N})(N^c - 1)}
\end{align*}
and $(n_1, n_2, n_3, n_4)$ is an off-diagonal solution to the energy equation, then some $n_i$ is at most $N^{1 - \delta(N, c)}$.

Results in the estimate
\begin{align*}
    E([N]^c) = 2N^2 - N + O(N^{1 - \gamma})
\end{align*}
where
\begin{align*}
    \gamma < \frac{1}{2N^2(\log{N})(N^c - 1)}
\end{align*}

\subsection{}

With the previous technique we get $|n_1n_2 - n_3 n_4| \leq M$, say. Hence let $n_1 n_2 - n_3 n_4 = m$ for $|m| \leq M$.

Fix $n_1 > n_3$. Let $d = \gcd(n_1, n_3)$ which is a divisor of $m$. Let $n_1 = d a_1$ and $n_3 = d a_3$.

If $(n_1, A, n_3, B)$ and $(n_1, C, n_3, D)$ are two solutions to the system then
\begin{align*}
    a_1(A - C) = a_3 (B - D).
\end{align*}
It follows that $C = A + ta_3$ and $D = ta_1 + B$. Thus
\begin{align*}
    B^c - A^c =
    n_1^c - n_3^c =
    D^c - C^c =
    (ta_1 + B)^c - (ta_2 + A)^c.
\end{align*}


Solutions to this equation are given by
\begin{align*}
    (n_1, n_2, n_3, n_4) = (ma_1, a_2, ma_3, a_4)
\end{align*}
where $a_1 a_2 - a_3 a_4 = 1$, so it suffices to parameterise this. We have $a_1, a_3 \leq N/m, a_2, a_4 \leq N$ and $\gcd(a_1, a_3) = 1$ too.

Fix $(A, B) = (a_1, a_3)$. If $(a_2, a_4)$ and $(b_2, b_4)$ are two solutions, then
\begin{align*}
    A (a_2 - b_2) - B(a_4 - b_4) = 0.
\end{align*}
Then $a_4 - b_4 = A C$ so $a_2 - b_2 = B C$. It follows that every solution $(A, b_2, B, b_4)$ is
\begin{align*}
    (A, a_2, B, a_4) =
    (A, b_2 + BC, B, b_4 + AC).
\end{align*}
Now
\begin{align*}
    n_1^c + n_2^c - n_3^c - n_4^c &=
    m^c a_1^c + a_2^c - m^c a_3^c - a_4^c
    \\ &=
    m^c A^c + (b_2 + BC)^c - m^c B^c - (b_4 + AC)^c
    \\ &=
    m^c (A^c - B^c) + (b_2 + BC)^c - (b_4 + AC)^c.
\end{align*}
Now
\begin{align*}
    (b_2 + BC)^c - (BC)^c = b_2 c \xi^{c - 1}
    \leq cN^c
\end{align*}
hence
\begin{align*}
    (m^c - C^c) (A^c - B^c) \ll cN^c.
\end{align*}

==> article/content2/GAPs.tex <==
\section{GAPs}

\textbf{This is an experimental section where I try to do GAPs.}

In this section we prove the following theorem.

\begin{manualtheorem}{C}
    Let $P$ be a generalised arithmetic progression of rank $r$ and cardinality $N$ in $\R_{\geq 0}$. Then for each $b \in \R_{\geq 0}$
    \begin{align*}
        \left|
        \left\{
        (a_1, \dots, a_k) \in P^k :
        a_1^c + \dots + a_k^c = b
        \right\}
        \right|
        \ll_{\eps, k, r} N^\eps.
    \end{align*}
    In particular, the big-$O$ constant does not depend on $c$ or $b$.
\end{manualtheorem}

Suppose $P$ has the form
\begin{align*}
    \{\alpha + \beta_1 n_1 + \dots + \beta_r n_r : n_i \in [L_i]\}.
\end{align*}
We can assume that the GAP is proper, in which case $N = L_1 \dots L_r$ and the coordinates of $\vec{\beta}$ are $\Q$-linearly independent. As in Section \ref{proof_of_theorem_B}, we will use definable families to achieve uniformity in the parameters $c, \alpha, \vec{\beta}$ and $b$. Thus let $\Lambda = \R \times \R_{\geq 0} \times \R_{>0}^r \times \R_{\geq 0}$ and let
\begin{align*}
    X = \{(c, \alpha, \vec{\beta}, b, \vec{x}_1, \dots, \vec{x}_k) \in \Lambda \times \R_{>0}^{rk} :
    (\alpha + \vec{\beta} \cdot \vec{x}_1)^c + \dots +
    (\alpha + \vec{\beta} \cdot \vec{x}_k)^c = b
    \},
\end{align*}
which becomes an $\R_{\exp}$-definable family with the projection $X \to \Lambda$.

Let $\lambda = (c, \alpha, \vec{\beta}, b) \in \Lambda$. For $(\xi_1, \dots, \xi_k) \in \R_{>0}^k$ satisfying
\begin{align*}
    \xi_1^c + \dots + \xi_k^c = b,
\end{align*}
the semi-algebraic subset $T(\vec{\xi})$ of $X_\lambda$ defined by
\begin{align*}
    \alpha + \beta \cdot \vec{x}_i = \xi_i
\end{align*}
for $i \in \{1, \dots, k\}$ can contain at most one rational point. This is because the coordinates of $\beta$ are $\Q$-linearly independent. Also every rational point is contained in a unique $T(\vec{\xi})$.

By (a counting result) the set $X_\lambda(\Q, N)$ is contained in at most $O_X(N^\eps)$ basic blocks. Hence there are at most $O_{k, r}(N^\eps)$ rational points of height at most $N$.

\section{GAPs in algebraic numbers}

Suppose $A$ lies in the GAP
\begin{align*}
    P = \{\alpha + n_1 \beta_1 + \dots + n_r \beta_r : n_i \leq N_i\},
\end{align*}
where $\beta_1, \dots, \beta_r$ are algebraic numbers.

Let $\gamma = n_1 \beta_1 + \dots + n_r \beta_r$. Then if $\gamma \in K$ then
\begin{align*}
    H(\gamma) =
    \sum_{v \in \Sigma_K} 
    \frac{n_v}{[K : \Q]}
    \max(1, |\gamma|_v)
    \geq 
    \frac{n_v}{[K : \Q]}
    \max(1, |\gamma|_v)
\end{align*}
for any $v \in \Sigma_K$. We have to show that roughly the height of $\gamma$ grows with $\max\{|n_i|\}$ and $H(\beta)$.

\subsection{Rank two GAPs}

Let $A$ be a subset of the proper GAP 
\begin{align*}
    P = \{\alpha + \beta m + \gamma n : 
    m \in [M], n \in [N]
    \}.
\end{align*}
Hence $\beta, \gamma$ are linearly independent over $\Q$ and $MN = |P|$.

For each $a \in A$, consider the set
\begin{align*}
    X_{a, c} = \{(x_1, x_2, x_3) \in \R^3 :
    x_1^c + x_2^c = x_3^c + a^c\},
\end{align*}
which we can consider as a fibre in an $\R_{\exp}$-definable family. Consider the map
\begin{align*}
    T : \R^6 &\to \R^3 \\
    (m_1, n_1, m_2, n_2, m_3, n_3) &\mapsto
    (\alpha + m_1 \beta + n_1 \gamma, 
    \alpha + m_2 \beta + n_2 \gamma,
    \alpha + m_3 \beta + n_3 \gamma
    )
\end{align*}
and let $Y_{a, c} = T^{-1}(X_{a, c}) \subseteq \R^6$.

\begin{lemma}
    Let $Z \subseteq Y_{a, c}$ be an irreducible semi-algebraic subset of positive dimension. Then $Z$ is defined by an equation of the form
    \begin{align}
    \label{trivial_semi-algebraic_sets}
        m_i \beta + n_i \gamma = m_3 \beta + n_3 \gamma,
    \end{align}
    for $i \in \{1, 2\}$, or is defined by the three equations
    \begin{align}
    \label{non-trivial_semi-algebraic_sets}
        \alpha + m_j \beta + n_j \gamma = \xi_j 
    \end{align}
    for $j \in \{1, 2, 3\}$, where $(\xi_1, \xi_2, \xi_3) \in X_{a, c}$.
\end{lemma}
\begin{proof}
    The set $T(Z)$ is an irreducible semi-algebraic subset of $X_{a, c}$. Hence $T(Z)$ is given by $x_1 = x_3$, or $x_2 = x_3$, or is a point. The statement follows.
\end{proof}

The semi-algebraic sets of the form (\ref{trivial_semi-algebraic_sets}) do not trouble us, for they only contribute to the trivial solutions of the additive energy equation. On the other hand, every rational point on $Y_{a, c}$ is contained in a semi-algebraic subset of type (\ref{non-trivial_semi-algebraic_sets}) for some $(\xi_1, \xi_2, \xi_3)$. Since $\beta, \gamma$ are assumed linearly independent over $\Q$, each of these non-trivial semi-algebraic sets can contain an most one rational point.

Suppose, without loss of generality, that $N \leq |P|^{1/2}$. Consider a pair $(n_1, n_2) \in [N]^2$, and the map $\pi_{n_1, n_2} : \R^4 \to \R^2$ projecting from $\R^6$ with $n_1, n_2$ fixed (hence $\R^4$) onto the coordinates $(m_1, m_2)$ in $\R^2$. Consider $Z = Z_{a, c, n_1, n_2}$, which is the image of $Y_{a, c}$ under this map. Hence
\begin{align*}
    Z = 
    \left\{
    (m_1, m_2) \in \R^2 :
    \exists m_3, n_3 \in \R :
    (n_1, m_1, m_2, n_2, m_3, n_3) \in Y_{a, c}
        \right\}
\end{align*}
is definable in $\R_{\exp}$.

Let $S \subseteq Z$ be positive-dimensional, irreducible and semi-algebraic. Then $\pi^{-1}(S) \subseteq Y_{a, c}$ must be of the form (\ref{non-trivial_semi-algebraic_sets}) (the other kind of set doesn't matter). Since $n_1, n_2, \xi_1, \xi_2$ are constant on $S$, so is $m_1, m_2$. Hence $S$ is constant. This shows that $Z$ cannot contain semi-algebraic subsets of positive dimension. Thus by Pila--Wilkie
\begin{align*}
    |Z(\Q, M)| \ll (\log M)^{O(1)}.
\end{align*}
That is: if $n_1, n_2$ are fixed there are at most $(\log M)^{O(1)}$ possible $(m_1, m_2)$. Now $\xi_3$ is determined, and this determines $m_3, n_3$ uniquely. Hence:

\begin{theorem}
    The number of rational points on $Y_{a, c}$ that do not give trivial solutions to the additive energy equation is at most
    \begin{align*}
        N^2 (\log M)^{O(1)} \ll
        |P| (\log |P|)^{O(1)}.
    \end{align*}
\end{theorem}

\begin{corollary}
    We have
    \begin{align*}
        E(A^{[c]}) \ll 
        |A||P| (\log |P|)^{O(1)}.
    \end{align*}
    Thus if $A$ is a subset of a rank $2$ GAP with density $\alpha$ then
    \begin{align*}
        E(A^{[c]}) \ll_{\eps} \frac{|A|^{2 + \eps}}{\alpha^{1 + \eps}}.
    \end{align*}
\end{corollary}

==> article/frontmatter/body_formatting.tex <==
%auto-ignore

%this file is inputted to the main.tex file after all other frontmatter items have been inputted. Any formatting settings for the body of document can be put here

\pagenumbering{arabic}

%header footer
% \pagestyle{fancy}
% \fancyhead{}
% \fancyhead[L]{\nouppercase{\leftmark}}
% \fancyhead[R]{\nouppercase{\rightmark}}
% \fancyfoot{}
% \fancyfoot[C]{\thepage}
% \renewcommand{\headrulewidth}{0pt}
